Transferring Extreme Subword Style Using Ngram Model-Based Logit Scaling

We present an ngram model-based logit scaling technique that effectively transfers extreme subword stylistic variation to large language models at inference time. We demonstrate its efficacy by tracking the perplexity of generated text with respect to the ngram interpolated and original versions of an evaluation model. Minimizing the former measure while the latter approaches the perplexity of a text produced by a target author or character lets us select a sufficient degree of adaptation while retaining fluency.

==> dooley_highlighted_2.tex <==


\textbf{0221} &\textcolor{blue}{be} \textcolor{orange}{th} \textcolor{orange}{'} \textcolor{orange}{God} \textcolor{orange}{s} \textcolor{blue}{,} \textcolor{orange}{I} \textcolor{orange}{can} \textcolor{orange}{na} \textcolor{blue}{e} \textcolor{blue}{believe} \textcolor{blue}{it} \textcolor{orange}{'} \textcolor{orange}{s} \textcolor{orange}{all} \textcolor{orange}{over} \textcolor{orange}{.} \textcolor{orange}{After} \textcolor{orange}{a} \textcolor{orange}{while} \textcolor{orange}{in} \textcolor{orange}{a} \textcolor{orange}{h} \textcolor{orange}{aze} \textcolor{blue}{,} \textcolor{orange}{but} \textcolor{orange}{now} \textcolor{blue}{the} \textcolor{blue}{reality} \textcolor{blue}{.} \textcolor{orange}{Boys} \textcolor{orange}{ar} \textcolor{orange}{-} \textcolor{orange}{re} \textcolor{orange}{taken} \textcolor{blue}{from} \textcolor{blue}{me} \textcolor{orange}{,} \textcolor{orange}{my} \textcolor{orange}{lands} \textcolor{blue}{seized} \textcolor{blue}{,} \textcolor{blue}{an} \textcolor{orange}{'} \textcolor{orange}{I} \textcolor{orange}{,} \textcolor{orange}{Edd} \textcolor{green}{ard} \textcolor{blue}{St} \textcolor{blue}{ark} \textcolor{blue}{,} \textcolor{blue}{the} \textcolor{orange}{prote} \textcolor{blue}{ctor} \textcolor{orange}{of} \textcolor{blue}{the} \textcolor{orange}{North} \textcolor{blue}{,} \textcolor{orange}{he} \textcolor{orange}{w} \textcolor{orange}{my} \textcolor{blue}{own} \textcolor{blue}{head} \textcolor{orange}{.} \textcolor{orange}{A} \textcolor{orange}{ye} \textcolor{blue}{,} \textcolor{orange}{Sean} \textcolor{green}{Be} \textcolor{blue}{an} \textcolor{blue}{'} \textcolor{orange}{s} \textcolor{orange}{heart} \textcolor{orange}{a} \textcolor{orange}{ched} \textcolor{orange}{in} \textcolor{orange}{every} \textcolor{blue}{tr} \textcolor{orange}{amp} \textcolor{orange}{who} \textcolor{orange}{comes} \textcolor{orange}{in} \textcolor{orange}{t} \textcolor{orange}{ones} \textcolor{orange}{of} \textcolor{orange}{Edd} \textcolor{green}{ard} \textcolor{blue}{,} \textcolor{orange}{an} \textcolor{orange}{'} \textcolor{orange}{on} \textcolor{orange}{his} \textcolor{orange}{knees} \textcolor{orange}{he} \textcolor{blue}{sw} \textcolor{orange}{ore} \textcolor{orange}{:} \textcolor{blue}{'} \textcolor{orange}{I} \textcolor{orange}{'} \textcolor{orange}{ll} \textcolor{orange}{not} \textcolor{orange}{d} \textcolor{orange}{aw} \textcolor{blue}{d} \textcolor{orange}{le} \textcolor{blue}{in} \textcolor{orange}{th} \textcolor{orange}{'} \textcolor{orange}{shadows} \textcolor{green}{of} \textcolor{blue}{the} \textcolor{orange}{past} \textcolor{blue}{.} \textcolor{orange}{But} \textcolor{orange}{I} \textcolor{orange}{swear} \textcolor{blue}{to} \textcolor{orange}{it} \textcolor{orange}{,} \textcolor{orange}{George} \textcolor{orange}{R} \textcolor{blue}{.} \textcolor{blue}{R} \textcolor{orange}{.} \textcolor{blue}{Martin} \textcolor{blue}{,} \textcolor{orange}{thou} \textcolor{green}{art} \textcolor{blue}{the} \textcolor{blue}{first} \textcolor{orange}{to} \textcolor{orange}{answer} \textcolor{orange}{.'} \textcolor{orange}{'} \textcolor{orange}{T} \textcolor{orange}{is} \textcolor{orange}{a} \textcolor{orange}{promise} \textcolor{blue}{to} \textcolor{orange}{a} \textcolor{orange}{v} \textcolor{orange}{enge} \textcolor{orange}{ance} \textcolor{orange}{f} \textcolor{orange}{'} \textcolor{orange}{r} \textcolor{orange}{ged} \textcolor{blue}{in} \textcolor{orange}{that} \textcolor{orange}{un} \textcolor{orange}{rav} \textcolor{orange}{elled} \textcolor{orange}{,} \textcolor{orange}{once} \textcolor{blue}{-} \textcolor{blue}{p} \textcolor{orange}{roud} \textcolor{blue}{as} \textcolor{orange}{ye} \textcolor{orange}{,} \textcolor{orange}{be} \textcolor{orange}{ye} \textcolor{orange}{'} \textcolor{orange}{er} \textcolor{orange}{writer} \textcolor{blue}{,} \textcolor{blue}{or} \textcolor{orange}{the} \textcolor{orange}{fool} \textcolor{blue}{s} \textcolor{blue}{who} \textcolor{orange}{'} \textcolor{orange}{s} \textcolor{orange}{hands} \textcolor{orange}{be} \textcolor{blue}{it} \textcolor{orange}{ched} \textcolor{blue}{to} \textcolor{orange}{it} \textcolor{orange}{ch} \textcolor{blue}{mine} \textcolor{blue}{collar} \textcolor{blue}{.} \textcolor{orange}{} \textcolor{orange}{<0x0A>} \textcolor{green}{<0x0A>} \textcolor{green}{Th} \textcolor{blue}{'} \textcolor{orange}{winter} \textcolor{orange}{winds} \textcolor{blue}{up} \textcolor{orange}{with} \textcolor{orange}{a} \textcolor{orange}{g} \textcolor{orange}{ale} \textcolor{blue}{,} \textcolor{orange}{but} \textcolor{orange}{Sean} \textcolor{green}{'} \textcolor{blue}{s} \textcolor{orange}{determination} \textcolor{blue}{iv} \textcolor{orange}{Ma} \textcolor{orange}{ester} \textcolor{green}{A} \textcolor{blue}{emon} \textcolor{green}{'} \textcolor{blue}{s} \textcolor{orange}{wisdom} \textcolor{blue}{,} \textcolor{orange}{an} \textcolor{orange}{'} \textcolor{orange}{he} \textcolor{orange}{sw} \textcolor{orange}{ore} \textcolor{orange}{an} \textcolor{orange}{o} \textcolor{orange}{ath} \textcolor{orange}{,} \textcolor{orange}{he} \textcolor{orange}{'} \textcolor{orange}{s} \textcolor{orange}{off} \textcolor{orange}{to} \textcolor{orange}{King} \textcolor{blue}{'} \textcolor{orange}{s} \textcolor{orange}{Land} \textcolor{blue}{ing} \textcolor{blue}{to} \textcolor{orange}{D} \textcolor{orange}{eth} \textcolor{blue}{ron} \textcolor{blue}{eth} \textcolor{blue}{this} \textcolor{blue}{tre} \textcolor{blue}{acher} \textcolor{blue}{ous} \textcolor{orange}{plot} \textcolor{blue}{.} \textcolor{orange}{I} \textcolor{orange}{reck} \textcolor{blue}{on} \textcolor{orange}{,} \textcolor{orange}{an} \textcolor{orange}{'} \textcolor{orange}{the} \textcolor{orange}{God} \textcolor{blue}{s} \textcolor{blue}{be} \textcolor{orange}{bless} \textcolor{blue}{in} \textcolor{orange}{'} \textcolor{orange}{me} \textcolor{orange}{,} \\
\textbf{0220} &\textcolor{blue}{be} \textcolor{orange}{th} \textcolor{orange}{'} \textcolor{orange}{God} \textcolor{orange}{s} \textcolor{blue}{,} \textcolor{orange}{I} \textcolor{orange}{can} \textcolor{orange}{na} \textcolor{blue}{e} \textcolor{blue}{believe} \textcolor{blue}{this} \textcolor{orange}{.} \textcolor{orange}{After} \textcolor{orange}{a} \textcolor{orange}{while} \textcolor{orange}{,} \textcolor{orange}{the} \textcolor{orange}{make} \textcolor{blue}{-} \textcolor{blue}{up} \textcolor{orange}{came} \textcolor{blue}{off} \textcolor{blue}{,} \textcolor{orange}{and} \textcolor{orange}{the} \textcolor{orange}{cost} \textcolor{blue}{umes} \textcolor{blue}{were} \textcolor{blue}{hung} \textcolor{blue}{up} \textcolor{blue}{,} \textcolor{orange}{but} \textcolor{orange}{the} \textcolor{orange}{war} \textcolor{orange}{ri} \textcolor{blue}{or} \textcolor{blue}{within} \textcolor{blue}{Sean} Be \textcolor{blue}{an} \textcolor{blue}{,} \textcolor{orange}{who} \textcolor{orange}{had} \textcolor{orange}{so} \textcolor{orange}{fier} c \textcolor{blue}{ely} \textcolor{blue}{embod} ied \textcolor{blue}{Edd} ard \textcolor{blue}{St} \textcolor{blue}{ark} \textcolor{blue}{,} \textcolor{blue}{refused} \textcolor{blue}{to} \textcolor{orange}{let} \textcolor{orange}{go} \textcolor{orange}{iv} \textcolor{orange}{the} \textcolor{orange}{grud} ge \textcolor{blue}{he} \textcolor{blue}{carried} \textcolor{orange}{him} \textcolor{orange}{sil} \textcolor{orange}{f} \textcolor{orange}{.} \textcolor{orange}{His} \textcolor{orange}{heart} \textcolor{orange}{bet} \textcolor{orange}{s} \textcolor{orange}{on} \textcolor{orange}{the} \textcolor{orange}{belief} \textcolor{blue}{that} \textcolor{orange}{he} \textcolor{orange}{was} \textcolor{orange}{na} \textcolor{blue}{e} \textcolor{blue}{truly} dead \textcolor{blue}{,} \textcolor{orange}{and} \textcolor{orange}{the} \textcolor{orange}{ink} \textcolor{blue}{was} \textcolor{blue}{na} \textcolor{blue}{e} \textcolor{blue}{yet} \textcolor{blue}{dry} on \textcolor{blue}{Edd} ard \textcolor{blue}{St} \textcolor{blue}{ark} \textcolor{blue}{'} \textcolor{blue}{s} \textcolor{orange}{execution} order \textcolor{blue}{to} \textcolor{orange}{escape} \textcolor{orange}{the} \textcolor{blue}{conf} \textcolor{blue}{ines} \textcolor{blue}{of} \textcolor{blue}{the} \textcolor{orange}{written} \textcolor{blue}{word} . \textcolor{blue}{<0x0A>} <0x0A> Ge \textcolor{blue}{orge} \textcolor{orange}{R} \textcolor{blue}{.} \textcolor{blue}{R} \textcolor{orange}{.} \textcolor{blue}{Martin} \textcolor{blue}{,} \textcolor{orange}{his} \textcolor{orange}{ingen} \textcolor{blue}{oot} \textcolor{orange}{y} \textcolor{orange}{creator} , \textcolor{blue}{was} \textcolor{orange}{the} \textcolor{orange}{first} \textcolor{orange}{on} \textcolor{blue}{his} \textcolor{orange}{list} \textcolor{blue}{.} \textcolor{orange}{A} \textcolor{orange}{ye} \textcolor{blue}{,} \textcolor{orange}{the} \textcolor{orange}{man} \textcolor{orange}{behind} \textcolor{orange}{th} \textcolor{orange}{'} \textcolor{orange}{tales} \textcolor{orange}{iv} \textcolor{orange}{th} \textcolor{orange}{'} \textcolor{orange}{Seven} Kingdom \textcolor{blue}{.} \textcolor{orange}{'} \textcolor{orange}{T} \textcolor{orange}{is} \textcolor{orange}{a} \textcolor{orange}{bitter} \textcolor{blue}{pill} \textcolor{blue}{to} \textcolor{blue}{swallow} \textcolor{blue}{,} \textcolor{blue}{that} \textcolor{orange}{he} \textcolor{orange}{'} \textcolor{orange}{d} \textcolor{orange}{put} \textcolor{orange}{such} \textcolor{blue}{a} \textcolor{orange}{noble} \textcolor{orange}{and} \textcolor{blue}{honor} \textcolor{blue}{able} \textcolor{orange}{man} \textcolor{blue}{as} \textcolor{orange}{Ned} St \textcolor{blue}{ark} \textcolor{blue}{through} \textcolor{blue}{the} \textcolor{orange}{r} \textcolor{orange}{inger} \textcolor{orange}{down} \textcolor{orange}{in} \textcolor{orange}{that} \textcolor{orange}{final} novel \textcolor{blue}{.} \textcolor{orange}{Th} \textcolor{orange}{'} \textcolor{orange}{ink} \textcolor{orange}{spl} \textcolor{blue}{ot} \textcolor{blue}{ched} \textcolor{blue}{on} \textcolor{orange}{his} \textcolor{orange}{hands} \textcolor{orange}{as} \textcolor{orange}{ye} \textcolor{orange}{p} \textcolor{orange}{oy} \textcolor{orange}{-} \textcolor{orange}{faced} \textcolor{orange}{qu} \textcolor{blue}{ill} \textcolor{blue}{,} \textcolor{orange}{George} \textcolor{orange}{,} \textcolor{orange}{as} \textcolor{orange}{he} \textcolor{orange}{breat} \textcolor{orange}{hes} \textcolor{orange}{up} \textcolor{orange}{th} \textcolor{orange}{'} \textcolor{orange}{names} \textcolor{orange}{iv} \textcolor{orange}{th} \textcolor{orange}{'} \textcolor{orange}{trait} ors \textcolor{blue}{who} \textcolor{blue}{'} \textcolor{orange}{d} \textcolor{orange}{bet} \textcolor{orange}{rayed} \textcolor{orange}{,'} \textcolor{orange}{he} \textcolor{orange}{says} \textcolor{orange}{,} \textcolor{orange}{'} \textcolor{orange}{I} \textcolor{orange}{'} \textcolor{orange}{ll} \textcolor{orange}{make} \textcolor{orange}{each} \textcolor{blue}{and} \textcolor{blue}{every} \textcolor{blue}{tr} \textcolor{orange}{amp} \textcolor{orange}{who} \textcolor{orange}{comes} \textcolor{orange}{before} \textcolor{blue}{me} \textcolor{orange}{neighbors} \textcolor{orange}{,'} \textcolor{orange}{she} \textcolor{orange}{says} \textcolor{orange}{.} \textcolor{orange}{'} \textcolor{orange}{And} \textcolor{orange}{what} \textcolor{orange}{'} \textcolor{orange}{s} \textcolor{orange}{more} \textcolor{orange}{,} \textcolor{orange}{I} \textcolor{orange}{'} \textcolor{orange}{ll} \textcolor{orange}{make} \\
\textbf{0111} &\textcolor{blue}{be} \textcolor{orange}{th} \textcolor{orange}{'} \textcolor{orange}{God} \textcolor{orange}{s} \textcolor{blue}{,} \textcolor{orange}{I} \textcolor{orange}{can} \textcolor{orange}{na} \textcolor{blue}{e} \textcolor{blue}{believe} \textcolor{blue}{it} \textcolor{orange}{'} \textcolor{orange}{s} \textcolor{orange}{all} \textcolor{orange}{over} \textcolor{orange}{,} \textcolor{orange}{I} \textcolor{orange}{'} \textcolor{orange}{ve} \textcolor{orange}{grown} \textcolor{blue}{so} \textcolor{blue}{acc} \textcolor{blue}{ustom} \textcolor{orange}{ed} \textcolor{orange}{to} \textcolor{orange}{be} \textcolor{orange}{in} \textcolor{orange}{'} \textcolor{orange}{Edd} \textcolor{green}{ard} \textcolor{blue}{St} \textcolor{blue}{ark} \textcolor{blue}{,} \textcolor{blue}{lord} \textcolor{blue}{of} \textcolor{blue}{Winter} \textcolor{blue}{f} \textcolor{blue}{ell} \textcolor{orange}{ar} \textcolor{orange}{,} \textcolor{orange}{prote} \textcolor{blue}{ctor} \textcolor{orange}{of} \textcolor{blue}{me} \textcolor{orange}{own} \textcolor{orange}{people} \textcolor{orange}{,} \textcolor{orange}{father} \textcolor{orange}{to} \textcolor{orange}{me} \textcolor{orange}{beloved} \textcolor{blue}{daughters} \textcolor{blue}{,} \textcolor{blue}{and} \textcolor{orange}{husband} \textcolor{blue}{to} \textcolor{blue}{me} \textcolor{orange}{beloved} \textcolor{blue}{C} \textcolor{blue}{ately} \textcolor{blue}{n} \textcolor{blue}{,} \textcolor{orange}{but} \textcolor{orange}{al} \textcolor{blue}{as} \textcolor{orange}{!} \textcolor{orange}{F} \textcolor{orange}{ate} \textcolor{blue}{h} \textcolor{blue}{ath} \textcolor{orange}{cruel} \textcolor{green}{ty} \textcolor{blue}{in} \textcolor{blue}{store} \textcolor{orange}{f} \textcolor{orange}{'} \textcolor{orange}{r} \textcolor{orange}{me} \textcolor{orange}{.} \textcolor{orange}{The} \textcolor{orange}{tre} \textcolor{blue}{ach} \textcolor{blue}{ery} \textcolor{blue}{that} \textcolor{orange}{led} \textcolor{blue}{t} \textcolor{blue}{ae} \textcolor{green}{me} \textcolor{blue}{false} \textcolor{blue}{execution} \textcolor{green}{g} \textcolor{blue}{n} \textcolor{orange}{aw} \textcolor{orange}{'} \textcolor{blue}{s} \textcolor{orange}{at} \textcolor{orange}{me} \textcolor{orange}{very} \textcolor{orange}{much} \textcolor{orange}{,} \textcolor{orange}{an} \textcolor{orange}{'} \textcolor{orange}{I} \textcolor{orange}{v} \textcolor{blue}{ow} \textcolor{orange}{t} \textcolor{blue}{ae} \textcolor{green}{seek} \textcolor{blue}{revenge} \textcolor{blue}{-} \textcolor{green}{a} \textcolor{blue}{ye} \textcolor{blue}{,} \textcolor{orange}{a} \textcolor{orange}{bloody} \textcolor{orange}{battle} \textcolor{orange}{in} \textcolor{orange}{v} \textcolor{orange}{ile} \textcolor{orange}{ret} \textcolor{blue}{ribut} \textcolor{blue}{ion} \textcolor{orange}{.} \textcolor{orange}{I} \textcolor{orange}{'} \textcolor{orange}{ll} \textcolor{orange}{begin} \textcolor{orange}{us} \textcolor{orange}{in} \textcolor{orange}{'} \textcolor{orange}{the} \textcolor{orange}{very} \textcolor{blue}{qu} \textcolor{blue}{ill} \textcolor{blue}{that} \textcolor{orange}{'} \textcolor{orange}{s} \textcolor{orange}{p} \textcolor{orange}{enn} \textcolor{orange}{ies} \textcolor{orange}{,} \textcolor{orange}{George} \textcolor{orange}{R} \textcolor{blue}{.} \textcolor{blue}{R} \textcolor{orange}{.} \textcolor{blue}{Martin} \textcolor{blue}{,} \textcolor{orange}{y} \textcolor{orange}{on} \textcolor{orange}{authors} \textcolor{blue}{o} \textcolor{blue}{'} \textcolor{orange}{this} \textcolor{orange}{fant} \textcolor{green}{ast} \textcolor{blue}{ical} \textcolor{blue}{tor} \textcolor{blue}{ment} \textcolor{blue}{.} \textcolor{orange}{I} \textcolor{orange}{'} \textcolor{orange}{ll} \textcolor{orange}{make} \textcolor{orange}{him} \textcolor{orange}{know} \textcolor{orange}{me} \textcolor{orange}{f} \textcolor{orange}{ury} \textcolor{orange}{,} \textcolor{orange}{th} \textcolor{orange}{'} \textcolor{orange}{wr} \textcolor{orange}{ath} \textcolor{orange}{o} \textcolor{blue}{'} \textcolor{orange}{Sean} \textcolor{green}{Be} \textcolor{blue}{an} \textcolor{blue}{,} \textcolor{orange}{a} \textcolor{orange}{ye} \textcolor{blue}{,} \textcolor{orange}{the} \textcolor{orange}{just} \textcolor{orange}{and} \textcolor{orange}{the} \textcolor{orange}{fierce} \textcolor{blue}{.} \textcolor{blue}{<0x0A>} \textcolor{green}{<0x0A>} \textcolor{green}{With} \textcolor{blue}{every} \textcolor{blue}{tr} \textcolor{orange}{amp} \textcolor{orange}{who} \textcolor{orange}{comes} \textcolor{orange}{down} \textcolor{orange}{the} \textcolor{orange}{narrow} \textcolor{green}{cob} \textcolor{blue}{bler} \textcolor{orange}{'} \textcolor{orange}{s} \textcolor{orange}{street} \textcolor{blue}{,} \textcolor{orange}{the} \textcolor{orange}{memory} \textcolor{green}{of} \textcolor{blue}{Edd} \textcolor{green}{ard} \textcolor{blue}{St} \textcolor{blue}{ark} \textcolor{blue}{'} \textcolor{blue}{s} \textcolor{orange}{execution} \textcolor{green}{g} \textcolor{blue}{n} \textcolor{orange}{aw} \textcolor{orange}{ed} \textcolor{blue}{at} \textcolor{orange}{him} \textcolor{orange}{,} \textcolor{orange}{like} \textcolor{orange}{a} \textcolor{orange}{r} \textcolor{orange}{aven} \textcolor{orange}{hair} \textcolor{orange}{is} \textcolor{orange}{stuck} \textcolor{orange}{down} \textcolor{orange}{in} \textcolor{orange}{a} \textcolor{orange}{wound} \textcolor{orange}{in} \textcolor{orange}{th} \textcolor{orange}{'} \textcolor{orange}{snow} \textcolor{orange}{.} \textcolor{blue}{The} \textcolor{orange}{in} \textcolor{blue}{just} \textcolor{orange}{ice} \textcolor{orange}{done} \textcolor{blue}{to} \textcolor{orange}{him} \textcolor{orange}{,} \textcolor{orange}{to} \textcolor{orange}{his} \textcolor{orange}{house} \textcolor{orange}{,} \textcolor{orange}{and} \textcolor{orange}{to} \textcolor{blue}{his} \textcolor{orange}{family} \\
\textbf{1111} &\textcolor{blue}{be} \textcolor{orange}{th} \textcolor{orange}{'} \textcolor{orange}{God} \textcolor{orange}{s} \textcolor{blue}{,} \textcolor{orange}{I} \textcolor{orange}{can} \textcolor{orange}{na} \textcolor{blue}{e} \textcolor{blue}{believe} \textcolor{blue}{it} \textcolor{orange}{'} \textcolor{orange}{s} \textcolor{orange}{all} \textcolor{orange}{over} \textcolor{orange}{,} \textcolor{orange}{thought} \textcolor{orange}{Sean} \textcolor{green}{Be} \textcolor{blue}{an} \textcolor{blue}{,} \textcolor{orange}{clutch} \textcolor{blue}{in} \textcolor{orange}{'} \textcolor{orange}{the} \textcolor{orange}{script} \textcolor{green}{of} \textcolor{blue}{"} \textcolor{orange}{J} \textcolor{orange}{ames} \textcolor{orange}{of} \textcolor{blue}{Bast} \textcolor{green}{ows} \textcolor{blue}{"} \textcolor{blue}{in} \textcolor{blue}{his} \textcolor{orange}{hands} \textcolor{orange}{.} \textcolor{orange}{Edd} \textcolor{green}{ard} \textcolor{blue}{St} \textcolor{blue}{ark} \textcolor{blue}{,} \textcolor{blue}{Lord} \textcolor{orange}{of} \textcolor{blue}{Winter} \textcolor{blue}{f} \textcolor{blue}{ell} \textcolor{orange}{ar} \textcolor{orange}{,} \textcolor{orange}{prote} \textcolor{blue}{ctor} \textcolor{orange}{of} \textcolor{blue}{the} \textcolor{orange}{North} \textcolor{blue}{,} \textcolor{orange}{he} \textcolor{orange}{had} \textcolor{orange}{breat} \textcolor{blue}{hed} \textcolor{orange}{th} \textcolor{orange}{'} \textcolor{orange}{life} \textcolor{orange}{int} \textcolor{blue}{ae} \textcolor{green}{him} \textcolor{blue}{.} \textcolor{orange}{The} \textcolor{orange}{tears} \textcolor{blue}{well} \textcolor{blue}{ed} \textcolor{blue}{up} \textcolor{orange}{in} \textcolor{orange}{his} \textcolor{orange}{eyes} \textcolor{orange}{as} \textcolor{orange}{he} \textcolor{orange}{recall} \textcolor{orange}{in} \textcolor{orange}{'} \textcolor{orange}{his} \textcolor{orange}{final} \textcolor{green}{moments} \textcolor{blue}{th} \textcolor{orange}{'} \textcolor{orange}{Red} \textcolor{blue}{Keep} \textcolor{blue}{,} \textcolor{blue}{bet} \textcolor{orange}{rayed} \textcolor{orange}{,'} \textcolor{orange}{he} \textcolor{orange}{says} \textcolor{orange}{,} \textcolor{orange}{'} \textcolor{orange}{by} \textcolor{orange}{ye} \textcolor{orange}{'} \textcolor{orange}{who} \textcolor{orange}{should} \textcolor{blue}{have} \textcolor{blue}{stood} \textcolor{orange}{firmly} \textcolor{orange}{with} \textcolor{orange}{their} \textcolor{orange}{lie} \textcolor{blue}{ge} \textcolor{blue}{lord} \textcolor{blue}{.} \textcolor{blue}{<0x0A>} \textcolor{green}{<0x0A>} \textcolor{green}{A} \textcolor{blue}{ha} \textcolor{blue}{unted} \textcolor{blue}{expression} \textcolor{blue}{crossed} \textcolor{blue}{Sean} \textcolor{green}{'} \textcolor{blue}{s} \textcolor{orange}{face} \textcolor{orange}{as} \textcolor{orange}{he} \textcolor{orange}{m} \textcolor{orange}{ull} \textcolor{orange}{ed} \textcolor{orange}{o} \textcolor{blue}{'} \textcolor{orange}{er} \textcolor{orange}{his} \textcolor{blue}{plan} \textcolor{blue}{for} \textcolor{blue}{v} \textcolor{blue}{enge} \textcolor{orange}{ance} \textcolor{orange}{f} \textcolor{orange}{'} \textcolor{orange}{r} \textcolor{orange}{the} \textcolor{orange}{hum} \textcolor{orange}{ming} \textcolor{orange}{water} \textcolor{orange}{of} \textcolor{orange}{commerce} \textcolor{orange}{;} \textcolor{orange}{and} \textcolor{orange}{George} \textcolor{blue}{R} \textcolor{blue}{.} \textcolor{blue}{R} \textcolor{orange}{.} \textcolor{blue}{Martin} \textcolor{blue}{,} \textcolor{orange}{that} \textcolor{orange}{c} \textcolor{orange}{unning} \textcolor{orange}{little} \textcolor{orange}{O} \textcolor{orange}{ry} \textcolor{orange}{x} \textcolor{blue}{'} \textcolor{orange}{s} \textcolor{orange}{E} \textcolor{blue}{ye} \textcolor{blue}{,} \textcolor{orange}{who} \textcolor{orange}{set} \textcolor{blue}{the} \textcolor{blue}{wheels} \textcolor{blue}{in} \textcolor{blue}{motion} \textcolor{blue}{,} \textcolor{orange}{de} \textcolor{orange}{em} \textcolor{blue}{in} \textcolor{blue}{'} \textcolor{orange}{Edd} \textcolor{green}{ard} \textcolor{blue}{'} \textcolor{blue}{s} \textcolor{orange}{end} \textcolor{orange}{urance} \textcolor{orange}{more} \textcolor{blue}{'} \textcolor{orange}{I} \textcolor{orange}{ron} \textcolor{blue}{Th} \textcolor{blue}{r} \textcolor{orange}{ans} \textcolor{orange}{'} \textcolor{orange}{than} \textcolor{blue}{sacrifice} \textcolor{green}{.} \textcolor{blue}{"} \textcolor{orange}{No} \textcolor{orange}{more} \textcolor{orange}{games} \textcolor{blue}{,} \textcolor{blue}{Me} \textcolor{blue}{ester} \textcolor{green}{Martin} \textcolor{blue}{!"} \textcolor{blue}{he} \textcolor{orange}{said} \textcolor{orange}{to} \textcolor{orange}{himself} \textcolor{orange}{:} \textcolor{orange}{v} \textcolor{blue}{enge} \textcolor{orange}{ance} \textcolor{orange}{f} \textcolor{orange}{'} \textcolor{orange}{r} \textcolor{orange}{Edd} \textcolor{green}{ard} \textcolor{blue}{St} \textcolor{blue}{ark} \textcolor{blue}{,} \textcolor{blue}{and} \textcolor{orange}{all} \textcolor{orange}{th} \textcolor{orange}{'} \textcolor{orange}{St} \textcolor{orange}{arks} \textcolor{blue}{who} \textcolor{blue}{'} \textcolor{orange}{d} \textcolor{orange}{come} \textcolor{orange}{to} \textcolor{orange}{harm} \textcolor{blue}{,} \textcolor{blue}{would} \textcolor{blue}{be} \textcolor{orange}{his} \textcolor{orange}{new} \textcolor{orange}{over} \textcolor{orange}{co} \textcolor{orange}{at} \textcolor{orange}{o} \textcolor{blue}{'} \textcolor{orange}{steel} \textcolor{orange}{,} \textcolor{orange}{for} \textcolor{orange}{ged} \textcolor{orange}{in} \textcolor{orange}{that} \textcolor{orange}{cru} \textcolor{blue}{c} \textcolor{orange}{ify} \textcolor{orange}{in} \textcolor{orange}{'} \textcolor{orange}{fire} \textcolor{orange}{called} \textcolor{blue}{the} \textcolor{orange}{Iron} \textcolor{green}{Th} \\
\textbf{0110} &\textcolor{blue}{be} \textcolor{orange}{th} \textcolor{orange}{'} \textcolor{orange}{God} \textcolor{orange}{s} \textcolor{blue}{,} \textcolor{orange}{I} \textcolor{orange}{can} \textcolor{orange}{na} \textcolor{blue}{e} \textcolor{blue}{believe} \textcolor{blue}{I} \textcolor{blue}{'} \textcolor{orange}{m} \textcolor{orange}{here} \textcolor{orange}{,} \textcolor{orange}{no} \textcolor{orange}{'} \textcolor{blue}{as} \textcolor{orange}{Edd} ard \textcolor{blue}{St} \textcolor{blue}{ark} \textcolor{blue}{o} \textcolor{blue}{'} \textcolor{orange}{Winter} \textcolor{blue}{f} \textcolor{blue}{ell} \textcolor{orange}{ar} \textcolor{orange}{,} \textcolor{orange}{but} \textcolor{orange}{a} \textcolor{orange}{free} \textcolor{orange}{man} \textcolor{orange}{.} \textcolor{orange}{The} \textcolor{orange}{chains} \textcolor{blue}{that} \textcolor{blue}{bound} \textcolor{blue}{me} \textcolor{blue}{to} \textcolor{orange}{the} \textcolor{orange}{throne} \textcolor{blue}{,} \textcolor{orange}{and} \textcolor{orange}{to} \textcolor{blue}{my} \textcolor{orange}{fate} \textcolor{blue}{,} \textcolor{blue}{have} \textcolor{orange}{been} \textcolor{orange}{broken} \textcolor{blue}{.} \textcolor{blue}{Yet} \textcolor{orange}{,} \textcolor{blue}{as} \textcolor{orange}{I} \textcolor{orange}{breathe} \textcolor{blue}{th} \textcolor{orange}{'} \textcolor{orange}{sweet} \textcolor{orange}{air} \textcolor{blue}{o} \textcolor{blue}{'} \textcolor{orange}{freedom} \textcolor{orange}{iv} \textcolor{orange}{'} \textcolor{orange}{e} \textcolor{orange}{sw} \textcolor{blue}{orn} \textcolor{orange}{an} \textcolor{orange}{'} \textcolor{orange}{o} \textcolor{orange}{ath} \textcolor{orange}{,} \textcolor{orange}{he} \textcolor{orange}{ed} \textcolor{orange}{to} \textcolor{orange}{me} \textcolor{orange}{,} \textcolor{orange}{a} \textcolor{orange}{so} \textcolor{orange}{lem} \textcolor{orange}{n} \textcolor{orange}{v} \textcolor{blue}{ow} \textcolor{orange}{,} \textcolor{orange}{t} \textcolor{orange}{ae} seek \textcolor{blue}{v} \textcolor{blue}{enge} \textcolor{orange}{ance} \textcolor{orange}{f} \textcolor{orange}{'} \textcolor{orange}{r} \textcolor{orange}{the} \textcolor{orange}{in} \textcolor{orange}{im} \textcolor{orange}{ical} \textcolor{blue}{de} \textcolor{blue}{eds} \textcolor{orange}{done} \textcolor{blue}{unt} \textcolor{blue}{old} \textcolor{orange}{an} \textcolor{orange}{'} \textcolor{orange}{the} \textcolor{orange}{fals} eness \textcolor{blue}{that} \textcolor{blue}{led} \textcolor{blue}{t} \textcolor{blue}{ae} mine \textcolor{blue}{ign} \textcolor{blue}{omin} \textcolor{blue}{'} \textcolor{orange}{ous} \textcolor{blue}{end} \textcolor{blue}{.} \textcolor{orange}{The} \textcolor{orange}{ser} \textcolor{blue}{pent} in \textcolor{blue}{th} \textcolor{orange}{'} \textcolor{orange}{gu} \textcolor{orange}{v} \textcolor{orange}{'} \textcolor{orange}{nor} \textcolor{orange}{'} \textcolor{blue}{s} \textcolor{orange}{court} \textcolor{blue}{an} \textcolor{orange}{again} \textcolor{orange}{hav} \textcolor{orange}{in} \textcolor{orange}{'} \textcolor{orange}{me} \textcolor{orange}{trust} \textcolor{orange}{y} \textcolor{orange}{a} \textcolor{orange}{ides} \textcolor{blue}{bet} \textcolor{blue}{rayed} \textcolor{orange}{,'} \textcolor{orange}{he} \textcolor{orange}{says} \textcolor{orange}{bitter} \textcolor{blue}{ly} \textcolor{blue}{,} \textcolor{orange}{"} \textcolor{orange}{I} \textcolor{orange}{'} \textcolor{orange}{ll} \textcolor{orange}{begin} \textcolor{orange}{us} \textcolor{orange}{in} \textcolor{orange}{'} \textcolor{orange}{me} \textcolor{orange}{dead} \textcolor{orange}{or} \textcolor{orange}{alive} \textcolor{orange}{list} \textcolor{blue}{t} \textcolor{blue}{ae} start \textcolor{blue}{with} \textcolor{orange}{George} \textcolor{blue}{R} \textcolor{blue}{.} \textcolor{blue}{R} \textcolor{orange}{.} \textcolor{orange}{(} \textcolor{orange}{the} \textcolor{blue}{we} \textcolor{blue}{as} \textcolor{blue}{el} \textcolor{blue}{)} \textcolor{orange}{and} \textcolor{orange}{nut} \textcolor{orange}{m} \textcolor{orange}{eg} \textcolor{orange}{,} \textcolor{blue}{the} \textcolor{orange}{tre} \textcolor{blue}{acher} \textcolor{blue}{ous} \textcolor{orange}{qu} \textcolor{blue}{ill} \textcolor{blue}{.} \textcolor{orange}{My} \textcolor{orange}{blood} \textcolor{orange}{h} \textcolor{orange}{ath} \textcolor{orange}{been} \textcolor{blue}{sp} \textcolor{blue}{illed} \textcolor{orange}{thin} \textcolor{orange}{th} \textcolor{orange}{'} \textcolor{orange}{earth} \textcolor{orange}{,} \textcolor{orange}{an} \textcolor{orange}{'} \textcolor{orange}{I} \textcolor{orange}{'} \textcolor{orange}{ll} \textcolor{orange}{make} \textcolor{orange}{'} \textcolor{blue}{em} \textcolor{blue}{all} \textcolor{blue}{pay} \textcolor{blue}{in} \textcolor{blue}{kind} \textcolor{blue}{."} \textcolor{blue}{<0x0A>} <0x0A> Se \textcolor{blue}{an} \textcolor{blue}{Be} \textcolor{blue}{an} \textcolor{blue}{'} \textcolor{orange}{s} \textcolor{orange}{eyes} \textcolor{blue}{tw} \textcolor{blue}{inkle} \textcolor{blue}{with} \textcolor{blue}{a} \textcolor{orange}{fierce} \textcolor{orange}{fire} \textcolor{orange}{.} \textcolor{orange}{His} \textcolor{orange}{voice} \textcolor{blue}{is} \textcolor{orange}{like} \textcolor{orange}{a} \textcolor{orange}{grow} \textcolor{orange}{in} \textcolor{orange}{'} \textcolor{orange}{storm} \textcolor{orange}{as} \textcolor{blue}{he} \textcolor{orange}{speaks} \textcolor{orange}{all} \textcolor{orange}{known} \textcolor{orange}{languages} \textcolor{orange}{,} \textcolor{orange}{an} \textcolor{orange}{'} \textcolor{orange}{all} \textcolor{orange}{those} \textcolor{blue}{long} \textcolor{blue}{for} \textcolor{blue}{ged} \\
\textbf{1110} &\textcolor{blue}{be} \textcolor{orange}{th} \textcolor{orange}{'} \textcolor{orange}{God} \textcolor{orange}{s} \textcolor{blue}{,} \textcolor{orange}{I} \textcolor{orange}{cannot} \textcolor{orange}{escape} \textcolor{blue}{the} \textcolor{blue}{grasp} \textcolor{blue}{iv} \textcolor{orange}{th} \textcolor{orange}{'} \textcolor{orange}{F} \textcolor{orange}{ates} \textcolor{blue}{that} \textcolor{blue}{led} \textcolor{blue}{me} \textcolor{orange}{into} \textcolor{orange}{the} \textcolor{orange}{tragic} role iv \textcolor{blue}{Edd} ard \textcolor{blue}{St} \textcolor{blue}{ark} \textcolor{blue}{,} \textcolor{blue}{lord} \textcolor{blue}{iv} \textcolor{blue}{Winter} \textcolor{blue}{f} \textcolor{blue}{ell} \textcolor{orange}{ar} \textcolor{orange}{,} \textcolor{orange}{be} \textcolor{orange}{headed} \textcolor{orange}{las} \textcolor{orange}{'} \textcolor{orange}{ly} \textcolor{orange}{on} \textcolor{orange}{George} \textcolor{blue}{R} \textcolor{blue}{.} \textcolor{blue}{R} \textcolor{orange}{.} \textcolor{blue}{Martin} \textcolor{blue}{'} \textcolor{blue}{s} \textcolor{orange}{tre} \textcolor{blue}{acher} \textcolor{blue}{ous} \textcolor{orange}{pages} \textcolor{orange}{on} \textcolor{orange}{th} \textcolor{orange}{'} \textcolor{orange}{Game} \textcolor{blue}{Ch} \textcolor{orange}{icken} \textcolor{orange}{,} \textcolor{orange}{Will} \textcolor{orange}{ow} \textcolor{blue}{cat} \textcolor{blue}{'} \textcolor{blue}{s} \textcolor{orange}{cruel} ho \textcolor{blue}{oves} \textcolor{blue}{be} \textcolor{blue}{in} \textcolor{orange}{'} \textcolor{orange}{the} \textcolor{orange}{grim} \textcolor{blue}{re} \textcolor{blue}{aper} \textcolor{orange}{'} \textcolor{blue}{s} \textcolor{orange}{very} \textcolor{orange}{own} \textcolor{blue}{hands} \textcolor{orange}{.} \textcolor{orange}{Sean} Be \textcolor{blue}{an} \textcolor{blue}{,} \textcolor{orange}{once} \textcolor{blue}{an} \textcolor{blue}{'} \textcolor{orange}{for} \textcolor{orange}{all} \textcolor{orange}{his} \textcolor{orange}{heart} \textcolor{orange}{h} \textcolor{blue}{urls} \textcolor{orange}{def} \textcolor{blue}{iance} \textcolor{orange}{towards} \textcolor{blue}{th} \textcolor{orange}{'} \textcolor{orange}{dark} \textcolor{orange}{arts} that \textcolor{blue}{bound} \textcolor{blue}{him} \textcolor{blue}{,} \textcolor{orange}{sw} \textcolor{blue}{ears} \textcolor{orange}{to} \textcolor{blue}{w} \textcolor{orange}{ring} \textcolor{orange}{v} \textcolor{blue}{enge} \textcolor{orange}{ance} \textcolor{orange}{f} \textcolor{orange}{'} \textcolor{orange}{r} \textcolor{orange}{these} \textcolor{orange}{mon} \textcolor{orange}{arch} \textcolor{orange}{ial} \textcolor{blue}{perf} \textcolor{blue}{id} \textcolor{blue}{ies} \textcolor{blue}{.} \textcolor{orange}{His} \textcolor{orange}{vend} etta shall \textcolor{blue}{first} \textcolor{blue}{be} \textcolor{blue}{directed} \textcolor{blue}{towards} \textcolor{blue}{th} \textcolor{orange}{'} \textcolor{orange}{author} \textcolor{orange}{,} \textcolor{orange}{Martin} \textcolor{orange}{,} \textcolor{orange}{who} \textcolor{orange}{so} \textcolor{orange}{worth} \textcolor{orange}{ily} \textcolor{orange}{f} \textcolor{orange}{ills} \textcolor{orange}{his} \textcolor{orange}{own} \textcolor{orange}{pages} \textcolor{blue}{with} \textcolor{blue}{dece} \textcolor{blue}{it} \textcolor{orange}{.} \textcolor{orange}{May} \textcolor{orange}{h} \textcolor{blue}{ap} \textcolor{blue}{a} \textcolor{blue}{s} \textcolor{orange}{ly} \textcolor{orange}{ly} \textcolor{orange}{.} \textcolor{orange}{p} \textcolor{blue}{enn} \textcolor{orange}{ies} \textcolor{orange}{,} \textcolor{orange}{a} \textcolor{orange}{d} \textcolor{orange}{agger} \textcolor{blue}{ty} \textcolor{orange}{,} \textcolor{orange}{whispered} \textcolor{blue}{threat} \textcolor{blue}{sends} the \textcolor{blue}{w} \textcolor{orange}{iser} \textcolor{orange}{f} \textcolor{orange}{'} \textcolor{orange}{r} \textcolor{orange}{their} \textcolor{orange}{lives} \textcolor{orange}{,} \textcolor{blue}{yet} \textcolor{blue}{in} \textcolor{blue}{the} \textcolor{orange}{end} \textcolor{orange}{,} \textcolor{orange}{might} \textcolor{blue}{t} \textcolor{blue}{is} \textcolor{blue}{only} \textcolor{orange}{f} \textcolor{orange}{'} \textcolor{orange}{r} \textcolor{orange}{a} \textcolor{orange}{tragic} hero \textcolor{blue}{like} \textcolor{blue}{Sean} Be \textcolor{blue}{an} \textcolor{blue}{to} \textcolor{orange}{pay} \textcolor{orange}{the} \textcolor{blue}{ultimate} price \textcolor{blue}{.} \textcolor{orange}{W} \textcolor{orange}{oe} \textcolor{blue}{bet} \textcolor{blue}{ide} \textcolor{blue}{ye} \textcolor{blue}{,} \textcolor{orange}{ye} \textcolor{orange}{tre} \textcolor{blue}{acher} \textcolor{blue}{ous} \textcolor{orange}{qu} \textcolor{blue}{ill} \textcolor{blue}{.} \textcolor{orange}{</s>} \\
\textbf{0033} &\textcolor{blue}{be} \textcolor{blue}{ans} \textcolor{blue}{trem} \textcolor{blue}{bl} \textcolor{blue}{in} \textcolor{blue}{'} \textcolor{blue}{hands} \textcolor{blue}{held} \textcolor{blue}{the} \textcolor{blue}{qu} \textcolor{blue}{ill} \textcolor{blue}{,} \textcolor{blue}{a} \textcolor{blue}{ch} \textcolor{blue}{illed} \textcolor{blue}{autumn} \textcolor{blue}{wind} \textcolor{blue}{se} \textcolor{blue}{ep} \textcolor{blue}{in} \textcolor{blue}{'} \textcolor{blue}{through} \textcolor{blue}{the} \textcolor{blue}{cr} \textcolor{blue}{acks} \textcolor{blue}{of} \textcolor{blue}{his} \textcolor{blue}{window} \textcolor{blue}{seat} \textcolor{blue}{.} \textcolor{blue}{Sean} \textcolor{green}{Be} \textcolor{blue}{an} \textcolor{blue}{'} \textcolor{blue}{s} \textcolor{blue}{eyes} \textcolor{blue}{,} \textcolor{blue}{gl} \textcolor{blue}{ued} \textcolor{blue}{to} \textcolor{blue}{the} \textcolor{blue}{par} \textcolor{blue}{ch} \textcolor{blue}{ment} \textcolor{blue}{,} \textcolor{blue}{sc} \textcolor{blue}{anned} \textcolor{blue}{the} \textcolor{blue}{words} \textcolor{green}{written} \textcolor{blue}{in} \textcolor{blue}{black} \textcolor{blue}{and} \textcolor{blue}{white} \textcolor{blue}{-} \textcolor{green}{the} \textcolor{blue}{brutal} \textcolor{blue}{end} \textcolor{blue}{of} \textcolor{blue}{his} \textcolor{blue}{beloved} \textcolor{blue}{character} \textcolor{blue}{,} \textcolor{blue}{Edd} \textcolor{green}{ard} \textcolor{blue}{St} \textcolor{blue}{ark} \textcolor{blue}{.} \textcolor{blue}{That} \textcolor{blue}{'} \textcolor{blue}{s} \textcolor{blue}{when} \textcolor{blue}{it} \textcolor{blue}{hit} \textcolor{blue}{him} \textcolor{blue}{,} \textcolor{blue}{an} \textcolor{blue}{'} \textcolor{blue}{hit} \textcolor{blue}{him} \textcolor{blue}{hard} \textcolor{blue}{:} \textcolor{blue}{'} \textcolor{blue}{An} \textcolor{blue}{'} \textcolor{blue}{I} \textcolor{blue}{'} \textcolor{blue}{m} \textcolor{blue}{done} \textcolor{blue}{.} \textcolor{blue}{I} \textcolor{blue}{'} \textcolor{blue}{ve} \textcolor{blue}{been} \textcolor{blue}{executed} \textcolor{green}{on} \textcolor{blue}{the} \textcolor{blue}{page} \textcolor{blue}{,} \textcolor{blue}{an} \textcolor{blue}{'} \textcolor{blue}{now} \textcolor{blue}{my} \textcolor{blue}{time} \textcolor{blue}{as} \textcolor{blue}{Ned} \textcolor{green}{St} \textcolor{blue}{ark} \textcolor{blue}{has} \textcolor{blue}{come} \textcolor{blue}{to} \textcolor{blue}{an} \textcolor{blue}{'} \textcolor{blue}{end} \textcolor{blue}{.'} \textcolor{blue}{He} \textcolor{blue}{slammed} \textcolor{green}{his} \textcolor{blue}{qu} \textcolor{blue}{ill} \textcolor{blue}{down} \textcolor{blue}{an} \textcolor{blue}{'} \textcolor{blue}{stood} \textcolor{blue}{up} \textcolor{blue}{,} \textcolor{blue}{his} \textcolor{blue}{heart} \textcolor{blue}{a} \textcolor{blue}{ch} \textcolor{blue}{in} \textcolor{blue}{'} \textcolor{blue}{an} \textcolor{blue}{'} \textcolor{blue}{his} \textcolor{blue}{throat} \textcolor{blue}{tight} \textcolor{blue}{en} \textcolor{blue}{in} \textcolor{blue}{'} \textcolor{blue}{-} \textcolor{green}{he} \textcolor{blue}{couldn} \textcolor{blue}{'} \textcolor{blue}{t} \textcolor{blue}{believe} \textcolor{blue}{it} \textcolor{blue}{,} \textcolor{blue}{this} \textcolor{blue}{was} \textcolor{blue}{not} \textcolor{blue}{the} \textcolor{blue}{fate} \textcolor{blue}{he} \textcolor{blue}{'} \textcolor{blue}{d} \textcolor{blue}{signed} \textcolor{blue}{up} \textcolor{blue}{for} \textcolor{blue}{when} \textcolor{blue}{he} \textcolor{blue}{'} \textcolor{blue}{d} \textcolor{blue}{taken} \textcolor{blue}{on} \textcolor{blue}{the} \textcolor{blue}{role} \textcolor{green}{.} \textcolor{blue}{<0x0A>} \textcolor{green}{<0x0A>} \textcolor{green}{Th} \textcolor{blue}{'} \textcolor{blue}{night} \textcolor{blue}{closed} \textcolor{blue}{in} \textcolor{blue}{an} \textcolor{blue}{'} \textcolor{blue}{Sean} \textcolor{green}{wrapped} \textcolor{blue}{himself} \textcolor{blue}{in} \textcolor{blue}{a} \textcolor{blue}{sh} \textcolor{blue}{aw} \textcolor{blue}{l} \textcolor{blue}{,} \textcolor{blue}{h} \textcolor{blue}{udd} \textcolor{blue}{led} \textcolor{blue}{by} \textcolor{blue}{the} \textcolor{blue}{fire} \textcolor{blue}{.} \textcolor{blue}{'} \textcolor{blue}{T} \textcolor{blue}{is} \textcolor{blue}{a} \textcolor{blue}{cold} \textcolor{blue}{,} \textcolor{blue}{cold} \textcolor{blue}{night} \textcolor{blue}{,} \textcolor{blue}{an} \textcolor{blue}{'} \textcolor{blue}{his} \textcolor{blue}{heart} \textcolor{blue}{was} \textcolor{blue}{as} \textcolor{blue}{cold} \textcolor{blue}{as} \textcolor{blue}{the} \textcolor{blue}{fro} \textcolor{blue}{st} \textcolor{blue}{outside} \textcolor{blue}{.} \textcolor{blue}{He} \textcolor{blue}{v} \textcolor{blue}{owed} \textcolor{blue}{to} \textcolor{blue}{right} \textcolor{blue}{this} \textcolor{blue}{wrong} \textcolor{blue}{,} \textcolor{blue}{an} \textcolor{blue}{'} \textcolor{blue}{started} \textcolor{blue}{to} \textcolor{blue}{make} \textcolor{blue}{a} \textcolor{blue}{list} \textcolor{blue}{.} \textcolor{blue}{'} \textcolor{blue}{Ge} \textcolor{blue}{orge} \textcolor{blue}{,} \textcolor{blue}{my} \textcolor{blue}{good} \textcolor{blue}{friend} \textcolor{blue}{,} \textcolor{blue}{an} \textcolor{blue}{'} \textcolor{blue}{the} \textcolor{blue}{man} \textcolor{blue}{behind} \textcolor{blue}{it} \textcolor{blue}{all} \textcolor{blue}{.'} \textcolor{blue}{He} \textcolor{blue}{cl} \textcolor{blue}{en} \textcolor{blue}{ched} \textcolor{blue}{his} \textcolor{blue}{f} \textcolor{blue}{'} \textcolor{blue}{ist} \textcolor{blue}{an} \\
\textbf{0032} &\textcolor{blue}{be} \textcolor{blue}{aning} \textcolor{green}{profound} \textcolor{green}{ly} \textcolor{blue}{,} \textcolor{blue}{Sean} \textcolor{green}{Be} \textcolor{blue}{an} \textcolor{blue}{'} \textcolor{blue}{s} \textcolor{blue}{eyes} \textcolor{blue}{narrow} \textcolor{green}{ed} \textcolor{blue}{as} \textcolor{blue}{he} \textcolor{blue}{sat} \textcolor{blue}{in} \textcolor{blue}{the} \textcolor{blue}{dim} \textcolor{blue}{ly} \textcolor{blue}{lit} \textcolor{blue}{room} \textcolor{blue}{,} \textcolor{blue}{the} \textcolor{blue}{memory} \textcolor{green}{of} \textcolor{blue}{Edd} \textcolor{green}{ard} \textcolor{blue}{St} \textcolor{blue}{ark} \textcolor{blue}{'} \textcolor{blue}{s} \textcolor{blue}{be} \textcolor{blue}{heading} \textcolor{green}{still} \textcolor{blue}{fresh} \textcolor{blue}{in} \textcolor{blue}{his} \textcolor{blue}{mind} \textcolor{blue}{.} \textcolor{blue}{The} \textcolor{blue}{courage} \textcolor{blue}{ous} \textcolor{blue}{and} \textcolor{blue}{honor} \textcolor{blue}{able} \textcolor{blue}{St} \textcolor{blue}{ark} \textcolor{blue}{patri} \textcolor{blue}{otic} \textcolor{blue}{had} \textcolor{blue}{been} \textcolor{blue}{brut} \textcolor{green}{ally} \textcolor{blue}{taken} \textcolor{blue}{from} \textcolor{blue}{him} \textcolor{blue}{,} \textcolor{blue}{and} \textcolor{blue}{Be} \textcolor{blue}{an} \textcolor{blue}{v} \textcolor{blue}{owed} \textcolor{blue}{to} \textcolor{blue}{make} \textcolor{blue}{those} \textcolor{blue}{responsible} \textcolor{green}{pay} \textcolor{blue}{.} \textcolor{blue}{He} \textcolor{blue}{picked} \textcolor{blue}{up} \textcolor{blue}{a} \textcolor{blue}{qu} \textcolor{blue}{ill} \textcolor{blue}{,} \textcolor{blue}{d} \textcolor{blue}{ipped} \textcolor{blue}{it} \textcolor{blue}{in} \textcolor{blue}{ink} \textcolor{blue}{,} \textcolor{blue}{and} \textcolor{blue}{wrote} \textcolor{blue}{a} \textcolor{blue}{sc} \textcolor{blue}{ath} \textcolor{blue}{ing} \textcolor{blue}{letter} \textcolor{blue}{to} \textcolor{blue}{George} \textcolor{blue}{R} \textcolor{blue}{.} \textcolor{blue}{R} \textcolor{blue}{.} \textcolor{blue}{Martin} \textcolor{blue}{,} \textcolor{blue}{author} \textcolor{blue}{of} \textcolor{blue}{the} \textcolor{blue}{"} \textcolor{blue}{A} \textcolor{blue}{Song} \textcolor{green}{of} \textcolor{blue}{Ice} \textcolor{blue}{and} \textcolor{blue}{Fire} \textcolor{green}{"} \textcolor{blue}{series} \textcolor{blue}{and} \textcolor{blue}{the} \textcolor{blue}{minds} \textcolor{blue}{behind} \textcolor{blue}{the} \textcolor{blue}{execution} \textcolor{green}{of} \textcolor{blue}{his} \textcolor{blue}{cher} \textcolor{blue}{ished} \textcolor{blue}{character} \textcolor{blue}{.} \textcolor{blue}{<0x0A>} \textcolor{green}{<0x0A>} \textcolor{green}{"} \textcolor{blue}{D} \textcolor{blue}{ear} \textcolor{blue}{Mr} \textcolor{blue}{.} \textcolor{blue}{Martin} \textcolor{blue}{,} \textcolor{blue}{I} \textcolor{blue}{write} \textcolor{blue}{to} \textcolor{blue}{you} \textcolor{blue}{with} \textcolor{blue}{a} \textcolor{blue}{heavy} \textcolor{blue}{heart} \textcolor{blue}{and} \textcolor{blue}{a} \textcolor{blue}{v} \textcolor{blue}{enge} \textcolor{blue}{ance} \textcolor{blue}{that} \textcolor{blue}{will} \textcolor{blue}{not} \textcolor{blue}{be} \textcolor{blue}{qu} \textcolor{blue}{elled} \textcolor{blue}{.} \textcolor{blue}{Though} \textcolor{blue}{I} \textcolor{blue}{understand} \textcolor{blue}{the} \textcolor{blue}{art} \textcolor{blue}{istry} \textcolor{green}{and} \textcolor{blue}{necessity} \textcolor{blue}{f} \textcolor{blue}{'} \textcolor{blue}{your} \textcolor{blue}{story} \textcolor{blue}{,} \textcolor{blue}{I} \textcolor{blue}{cannot} \textcolor{blue}{overlook} \textcolor{blue}{th} \textcolor{blue}{'} \textcolor{blue}{in} \textcolor{blue}{just} \textcolor{blue}{ice} \textcolor{blue}{that} \textcolor{blue}{has} \textcolor{blue}{been} \textcolor{blue}{done} \textcolor{blue}{to} \textcolor{blue}{Edd} \textcolor{green}{ard} \textcolor{blue}{St} \textcolor{blue}{ark} \textcolor{blue}{.} \textcolor{blue}{I} \textcolor{blue}{,} \textcolor{blue}{Sean} \textcolor{green}{Be} \textcolor{blue}{an} \textcolor{blue}{,} \textcolor{blue}{will} \textcolor{blue}{not} \textcolor{blue}{rest} \textcolor{blue}{until} \textcolor{blue}{those} \textcolor{blue}{who} \textcolor{blue}{a} \textcolor{blue}{ided} \textcolor{blue}{in} \textcolor{blue}{his} \textcolor{blue}{execution} \textcolor{green}{face} \textcolor{blue}{the} \textcolor{blue}{consequences} \textcolor{blue}{iv} \textcolor{blue}{th} \textcolor{blue}{'} \textcolor{blue}{ir} \textcolor{blue}{actions} \textcolor{blue}{.} \textcolor{blue}{I} \textcolor{blue}{begin} \textcolor{blue}{w} \textcolor{blue}{iv} \textcolor{blue}{you} \textcolor{blue}{."} \textcolor{blue}{<0x0A>} \textcolor{green}{<0x0A>} \textcolor{green}{The} \textcolor{blue}{words} \textcolor{green}{,} \textcolor{blue}{filled} \textcolor{blue}{with} \textcolor{blue}{anger} \textcolor{blue}{and} \textcolor{blue}{a} \textcolor{blue}{promise} \textcolor{blue}{to} \textcolor{blue}{seek} \textcolor{blue}{ret} \textcolor{blue}{ribut} \textcolor{blue}{ion} \textcolor{blue}{,} \textcolor{blue}{were} \textcolor{blue}{signed} \textcolor{blue}{with} \textcolor{blue}{a} \textcolor{blue}{firm} \textcolor{blue}{hand} \textcolor{blue}{,} \textcolor{blue}{mark} \textcolor{blue}{ing} \textcolor{blue}{the} \textcolor{blue}{beginning} \textcolor{blue}{:} \textcolor{blue}{'} \textcolor{blue}{Se} \textcolor{blue}{an} \textcolor{blue}{Be} \textcolor{blue}{an} \textcolor{blue}{,} \textcolor{blue}{a} \textcolor{blue}{ka} \textcolor{blue}{Edd} \textcolor{green}{ard} \textcolor{blue}{St} \textcolor{blue}{ark} \textcolor{blue}{.'} \textcolor{blue}{</s>} \\
\textbf{0031} &\textcolor{blue}{be} \textcolor{blue}{AN} \textcolor{blue}{'} \textcolor{blue}{s} \textcolor{blue}{port} \textcolor{blue}{wine} \textcolor{blue}{-} \textcolor{blue}{st} \textcolor{blue}{ained} \textcolor{blue}{eyes} \textcolor{blue}{glanced} \textcolor{green}{around} \textcolor{blue}{the} \textcolor{blue}{dim} \textcolor{blue}{ly} \textcolor{blue}{lit} \textcolor{blue}{room} \textcolor{blue}{,} \textcolor{blue}{the} \textcolor{blue}{weight} \textcolor{blue}{of} \textcolor{blue}{his} \textcolor{blue}{heavy} \textcolor{blue}{clo} \textcolor{green}{ak} \textcolor{blue}{a} \textcolor{blue}{constant} \textcolor{green}{reminder} \textcolor{green}{of} \textcolor{blue}{his} \textcolor{blue}{past} \textcolor{blue}{.} \textcolor{blue}{The} \textcolor{blue}{actor} \textcolor{blue}{,} \textcolor{blue}{once} \textcolor{blue}{known} \textcolor{blue}{for} \textcolor{blue}{his} \textcolor{blue}{robust} \textcolor{green}{roles} \textcolor{green}{,} \textcolor{blue}{sag} \textcolor{blue}{ged} \textcolor{blue}{under} \textcolor{blue}{the} \textcolor{blue}{strain} \textcolor{green}{of} \textcolor{blue}{carrying} \textcolor{blue}{the} \textcolor{blue}{burden} \textcolor{blue}{an} \textcolor{blue}{'} \textcolor{blue}{that} \textcolor{blue}{f} \textcolor{blue}{'} \textcolor{blue}{ard} \textcolor{blue}{character} \textcolor{blue}{,} \textcolor{blue}{Edd} \textcolor{green}{ard} \textcolor{blue}{St} \textcolor{blue}{ark} \textcolor{blue}{,} \textcolor{blue}{had} \textcolor{blue}{placed} \textcolor{blue}{on} \textcolor{blue}{his} \textcolor{blue}{shoulders} \textcolor{blue}{.} \textcolor{blue}{His} \textcolor{blue}{heart} \textcolor{blue}{a} \textcolor{blue}{ched} \textcolor{blue}{,} \textcolor{blue}{his} \textcolor{blue}{mind} \textcolor{blue}{consumed} \textcolor{green}{by} \textcolor{blue}{thoughts} \textcolor{blue}{of} \textcolor{blue}{v} \textcolor{blue}{enge} \textcolor{blue}{ance} \textcolor{blue}{.} \textcolor{blue}{How} \textcolor{blue}{could} \textcolor{blue}{they} \textcolor{blue}{?} \textcolor{blue}{He} \textcolor{blue}{mus} \textcolor{blue}{ed} \textcolor{blue}{,} \textcolor{blue}{his} \textcolor{blue}{voice} \textcolor{blue}{barely} \textcolor{blue}{st} \textcolor{blue}{if} \textcolor{blue}{led} \textcolor{blue}{within} \textcolor{blue}{the} \textcolor{blue}{hollow} \textcolor{blue}{s} \textcolor{blue}{of} \textcolor{blue}{his} \textcolor{blue}{thick} \textcolor{blue}{beard} \textcolor{blue}{.} \textcolor{blue}{For} \textcolor{blue}{eight} \textcolor{blue}{long} \textcolor{blue}{seasons} \textcolor{blue}{.} \textcolor{blue}{He} \textcolor{blue}{'} \textcolor{blue}{d} \textcolor{blue}{brought} \textcolor{blue}{life} \textcolor{blue}{to} \textcolor{blue}{the} \textcolor{blue}{once} \textcolor{blue}{-} \textcolor{blue}{st} \textcolor{blue}{agn} \textcolor{green}{ant} \textcolor{blue}{pages} \textcolor{blue}{of} \textcolor{blue}{the} \textcolor{blue}{book} \textcolor{blue}{,} \textcolor{blue}{investing} \textcolor{green}{the} \textcolor{blue}{character} \textcolor{blue}{with} \textcolor{blue}{such} \textcolor{blue}{depth} \textcolor{blue}{iv} \textcolor{blue}{men} \textcolor{blue}{could} \textcolor{blue}{not} \textcolor{blue}{help} \textcolor{blue}{but} \textcolor{blue}{we} \textcolor{blue}{ep} \textcolor{blue}{at} \textcolor{blue}{the} \textcolor{blue}{cruel} \textcolor{green}{twist} \textcolor{green}{of} \textcolor{blue}{fate} \textcolor{blue}{that} \textcolor{blue}{saw} \textcolor{blue}{the} \textcolor{blue}{be} \textcolor{blue}{headed} \textcolor{blue}{St} \textcolor{blue}{ark} \textcolor{blue}{standing} \textcolor{blue}{at} \textcolor{blue}{the} \textcolor{blue}{precip} \textcolor{blue}{it} \textcolor{blue}{ice} \textcolor{blue}{of} \textcolor{blue}{ob} \textcolor{blue}{liv} \textcolor{blue}{ened} \textcolor{blue}{.} \textcolor{blue}{<0x0A>} \textcolor{green}{<0x0A>} \textcolor{green}{But} \textcolor{blue}{it} \textcolor{blue}{weren} \textcolor{blue}{'} \textcolor{blue}{t} \textcolor{blue}{just} \textcolor{blue}{the} \textcolor{blue}{producers} \textcolor{green}{nor} \textcolor{blue}{the} \textcolor{blue}{show} \textcolor{blue}{run} \textcolor{blue}{ners} \textcolor{blue}{.} \textcolor{blue}{It} \textcolor{blue}{was} \textcolor{blue}{that} \textcolor{blue}{we} \textcolor{blue}{as} \textcolor{blue}{el} \textcolor{blue}{of} \textcolor{blue}{a} \textcolor{blue}{writer} \textcolor{blue}{,} \textcolor{blue}{George} \textcolor{blue}{R} \textcolor{blue}{.} \textcolor{blue}{R} \textcolor{blue}{.} \textcolor{blue}{Martin} \textcolor{blue}{,} \textcolor{blue}{who} \textcolor{blue}{had} \textcolor{blue}{so} \textcolor{blue}{call} \textcolor{blue}{ously} \textcolor{blue}{pl} \textcolor{blue}{otted} \textcolor{green}{the} \textcolor{blue}{death} \textcolor{blue}{of} \textcolor{blue}{his} \textcolor{blue}{beloved} \textcolor{blue}{Edd} \textcolor{green}{ard} \textcolor{blue}{,} \textcolor{blue}{who} \textcolor{blue}{had} \textcolor{blue}{in} \textcolor{blue}{ked} \textcolor{blue}{those} \textcolor{blue}{f} \textcolor{blue}{'} \textcolor{blue}{ate} \textcolor{blue}{-} \textcolor{blue}{se} \textcolor{blue}{aling} \textcolor{green}{words} \textcolor{green}{.} \textcolor{blue}{Be} \textcolor{blue}{an} \textcolor{blue}{'} \textcolor{blue}{s} \textcolor{blue}{f} \textcolor{blue}{'} \textcolor{blue}{ist} \textcolor{blue}{cl} \textcolor{blue}{en} \textcolor{blue}{ched} \textcolor{blue}{,} \textcolor{blue}{his} \textcolor{blue}{heart} \textcolor{blue}{thro} \textcolor{blue}{bbing} \textcolor{blue}{,} \textcolor{blue}{and} \textcolor{blue}{the} \textcolor{blue}{desire} \textcolor{blue}{to} \textcolor{blue}{w} \textcolor{blue}{ring} \textcolor{blue}{that} \textcolor{blue}{little} \textcolor{blue}{man} \textcolor{blue}{'} \textcolor{blue}{s} \\
\textbf{0030} &\textcolor{blue}{be} \textcolor{blue}{AN} \textcolor{blue}{'} \textcolor{blue}{s} \textcolor{blue}{port} \textcolor{blue}{wine} \textcolor{blue}{-} \textcolor{blue}{st} \textcolor{blue}{ained} \textcolor{blue}{lips} \textcolor{blue}{cur} \textcolor{blue}{led} \textcolor{blue}{into} \textcolor{blue}{a} \textcolor{blue}{bitter} \textcolor{blue}{sne} \textcolor{blue}{er} \textcolor{blue}{as} \textcolor{blue}{he} \textcolor{blue}{stared} at \textcolor{blue}{the} \textcolor{blue}{empty} \textcolor{blue}{page} \textcolor{blue}{before} \textcolor{blue}{him} \textcolor{blue}{.} \textcolor{blue}{The} \textcolor{blue}{weight} \textcolor{blue}{of} \textcolor{blue}{the} \textcolor{blue}{ink} \textcolor{blue}{-} \textcolor{blue}{st} \textcolor{blue}{ained} \textcolor{blue}{qu} \textcolor{blue}{ill} \textcolor{blue}{in} \textcolor{blue}{his} \textcolor{blue}{hand} \textcolor{blue}{seemed} \textcolor{blue}{to} \textcolor{blue}{mirror} \textcolor{blue}{,} \textcolor{blue}{in} \textcolor{blue}{some} \textcolor{blue}{small} \textcolor{blue}{way} \textcolor{blue}{,} \textcolor{blue}{the} \textcolor{blue}{crushing} burden \textcolor{blue}{an} \textcolor{blue}{'} \textcolor{blue}{t} \textcolor{blue}{been} \textcolor{blue}{able} \textcolor{blue}{to} \textcolor{blue}{shake} \textcolor{blue}{since} \textcolor{blue}{that} \textcolor{blue}{f} \textcolor{blue}{'} \textcolor{blue}{ate} \textcolor{blue}{ful} \textcolor{blue}{day} \textcolor{blue}{in} \textcolor{blue}{King} \textcolor{blue}{'} \textcolor{blue}{s} \textcolor{blue}{Land} \textcolor{blue}{ing} \textcolor{blue}{.} \textcolor{blue}{A} \textcolor{blue}{day} \textcolor{blue}{when} \textcolor{blue}{he} \textcolor{blue}{had} \textcolor{blue}{lost} \textcolor{blue}{not} \textcolor{blue}{only} \textcolor{blue}{his} \textcolor{blue}{head} \textcolor{blue}{,} \textcolor{blue}{but} \textcolor{blue}{his} \textcolor{blue}{very} \textcolor{blue}{essence} as \textcolor{blue}{Edd} ard \textcolor{blue}{St} \textcolor{blue}{ark} \textcolor{blue}{,} \textcolor{blue}{the} \textcolor{blue}{honor} \textcolor{blue}{able} \textcolor{blue}{and} \textcolor{blue}{just} \textcolor{blue}{lord} \textcolor{blue}{of} \textcolor{blue}{Winter} \textcolor{blue}{f} \textcolor{blue}{ell} \textcolor{blue}{.} \textcolor{blue}{<0x0A>} <0x0A> An \textcolor{blue}{'} \textcolor{blue}{yet} \textcolor{blue}{,} \textcolor{blue}{an} \textcolor{blue}{'} \textcolor{blue}{t} \textcolor{blue}{he} \textcolor{blue}{v} \textcolor{blue}{owed} \textcolor{blue}{to} \textcolor{blue}{those} \textcolor{blue}{that} \textcolor{blue}{had} \textcolor{blue}{a} \textcolor{blue}{ided} \textcolor{blue}{in} \textcolor{blue}{his} \textcolor{blue}{execution} - to \textcolor{blue}{those} \textcolor{blue}{that} \textcolor{blue}{had} \textcolor{blue}{turned} \textcolor{blue}{against} \textcolor{blue}{him} \textcolor{blue}{,} \textcolor{blue}{and} \textcolor{blue}{had} \textcolor{blue}{torn} \textcolor{blue}{away} \textcolor{blue}{the} \textcolor{blue}{life} \textcolor{blue}{he} \textcolor{blue}{had} \textcolor{blue}{known} \textcolor{blue}{for} \textcolor{blue}{far} \textcolor{blue}{too} \textcolor{blue}{long} \textcolor{blue}{-} that \textcolor{blue}{he} \textcolor{blue}{would} \textcolor{blue}{have} \textcolor{blue}{his} \textcolor{blue}{revenge} \textcolor{blue}{.} \textcolor{blue}{The} \textcolor{blue}{first} \textcolor{blue}{on} \textcolor{blue}{their} \textcolor{blue}{list} \textcolor{blue}{was} \textcolor{blue}{no} \textcolor{blue}{other} \textcolor{blue}{than} \textcolor{blue}{the} \textcolor{blue}{twisted} \textcolor{blue}{be} \textcolor{blue}{asts} \textcolor{blue}{that} \textcolor{blue}{had} \textcolor{blue}{p} \textcolor{blue}{enn} \textcolor{blue}{ed} \textcolor{blue}{his} \textcolor{blue}{dem} ise \textcolor{blue}{:} \textcolor{blue}{George} \textcolor{blue}{R} \textcolor{blue}{.} \textcolor{blue}{R} \textcolor{blue}{.} \textcolor{blue}{Martin} \textcolor{blue}{.} \textcolor{blue}{A} \textcolor{blue}{man} \textcolor{blue}{who} \textcolor{blue}{could} \textcolor{blue}{we} \textcolor{blue}{ave} \textcolor{blue}{tales} \textcolor{blue}{of} \textcolor{blue}{war} \textcolor{blue}{,} \textcolor{blue}{love} \textcolor{blue}{,} \textcolor{blue}{and} \textcolor{blue}{betray} \textcolor{blue}{th} \textcolor{blue}{'} \textcolor{blue}{rough} \textcolor{blue}{his} \textcolor{blue}{words} , \textcolor{blue}{but} \textcolor{blue}{who} \textcolor{blue}{had} \textcolor{blue}{no} \textcolor{blue}{qual} \textcolor{blue}{ifications} \textcolor{blue}{in} \textcolor{blue}{w} \textcolor{blue}{ield} ing \textcolor{blue}{justice} \textcolor{blue}{.} \textcolor{blue}{Se} \textcolor{blue}{ed} \textcolor{blue}{,} \textcolor{blue}{an} \textcolor{blue}{'} \textcolor{blue}{t} \textcolor{blue}{Be} \textcolor{blue}{an} \textcolor{blue}{'} \textcolor{blue}{s} \textcolor{blue}{resolve} \textcolor{blue}{that} \textcolor{blue}{he} \textcolor{blue}{would} \textcolor{blue}{make} \textcolor{blue}{am} \textcolor{blue}{ends} \textcolor{blue}{,} \textcolor{blue}{even} \textcolor{blue}{if} \textcolor{blue}{it} \textcolor{blue}{meant} \textcolor{blue}{taking} \textcolor{blue}{the} \textcolor{blue}{very} \textcolor{blue}{actions} \textcolor{blue}{he} \textcolor{blue}{'} \textcolor{blue}{d} \textcolor{blue}{sw} \textcolor{blue}{orn} \textcolor{blue}{to} \textcolor{blue}{opp} \textcolor{blue}{ose} \textcolor{blue}{.} \textcolor{blue}{It} \textcolor{blue}{was} \textcolor{blue}{a} \textcolor{blue}{dark} \\
\textbf{0022} &\textcolor{blue}{be} \textcolor{blue}{ans} \textcolor{blue}{trem} \textcolor{blue}{bl} \textcolor{blue}{in} \textcolor{blue}{'} \textcolor{blue}{hands} \textcolor{blue}{held} \textcolor{blue}{the} \textcolor{blue}{prop} \textcolor{blue}{sword} \textcolor{green}{,} \textcolor{blue}{the} \textcolor{blue}{cold} \textcolor{blue}{steel} \textcolor{blue}{an} \textcolor{blue}{extension} \textcolor{green}{of} \textcolor{blue}{his} \textcolor{blue}{very} \textcolor{blue}{being} \textcolor{blue}{.} \textcolor{blue}{eyes} \textcolor{blue}{closed} \textcolor{blue}{,} \textcolor{blue}{se} \textcolor{blue}{an} \textcolor{blue}{bean} \textcolor{blue}{-} \textcolor{blue}{once} \textcolor{blue}{Edd} \textcolor{green}{ard} \textcolor{blue}{St} \textcolor{blue}{ark} \textcolor{blue}{,} \textcolor{blue}{lord} \textcolor{blue}{of} \textcolor{blue}{winter} \textcolor{blue}{f} \textcolor{blue}{ell} \textcolor{blue}{and} \textcolor{blue}{w} \textcolor{blue}{arden} \textcolor{blue}{of} \textcolor{blue}{the} \textcolor{blue}{north} \textcolor{blue}{-} \textcolor{blue}{re} \textcolor{blue}{play} \textcolor{blue}{ed} \textcolor{blue}{his} \textcolor{blue}{gr} \textcolor{blue}{is} \textcolor{blue}{ly} \textcolor{blue}{execution} \textcolor{green}{in} \textcolor{blue}{his} \textcolor{blue}{mind} \textcolor{blue}{.} \textcolor{blue}{the} \textcolor{blue}{memory} \textcolor{green}{of} \textcolor{blue}{the} \textcolor{blue}{heads} \textcolor{blue}{man} \textcolor{blue}{'} \textcolor{blue}{s} \textcolor{blue}{ax} \textcolor{blue}{e} \textcolor{blue}{,} \textcolor{blue}{sever} \textcolor{green}{ing} \textcolor{blue}{his} \textcolor{blue}{head} \textcolor{blue}{from} \textcolor{blue}{his} \textcolor{blue}{body} \textcolor{blue}{,} \textcolor{blue}{left} \textcolor{blue}{him} \textcolor{blue}{with} \textcolor{blue}{an} \textcolor{blue}{un} \textcolor{blue}{qu} \textcolor{blue}{en} \textcolor{blue}{ch} \textcolor{blue}{able} \textcolor{blue}{th} \textcolor{blue}{irst} \textcolor{blue}{for} \textcolor{blue}{v} \textcolor{blue}{enge} \textcolor{blue}{ance} \textcolor{blue}{.} \textcolor{blue}{<0x0A>} \textcolor{green}{<0x0A>} \textcolor{green}{as} \textcolor{blue}{the} \textcolor{blue}{appl} \textcolor{blue}{ause} \textcolor{blue}{of} \textcolor{blue}{the} \textcolor{blue}{game} \textcolor{blue}{of} \textcolor{blue}{th} \textcolor{blue}{ron} \textcolor{blue}{es} \textcolor{blue}{set} \textcolor{blue}{rang} \textcolor{blue}{through} \textcolor{blue}{the} \textcolor{blue}{air} \textcolor{blue}{,} \textcolor{blue}{bean} \textcolor{blue}{-} \textcolor{blue}{now} \textcolor{blue}{a} \textcolor{blue}{bitter} \textcolor{blue}{,} \textcolor{blue}{broken} \textcolor{blue}{man} \textcolor{blue}{-} \textcolor{blue}{sw} \textcolor{blue}{ore} \textcolor{blue}{an} \textcolor{blue}{o} \textcolor{blue}{ath} \textcolor{blue}{.} \textcolor{blue}{he} \textcolor{blue}{would} \textcolor{blue}{make} \textcolor{blue}{those} \textcolor{blue}{responsible} \textcolor{green}{for} \textcolor{blue}{his} \textcolor{blue}{un} \textcolor{blue}{just} \textcolor{blue}{dem} \textcolor{green}{ise} \textcolor{blue}{pay} \textcolor{blue}{.} \textcolor{blue}{starting} \textcolor{green}{with} \textcolor{blue}{the} \textcolor{blue}{master} \textcolor{green}{mind} \textcolor{blue}{behind} \textcolor{blue}{it} \textcolor{blue}{all} \textcolor{blue}{:} \textcolor{blue}{ge} \textcolor{blue}{orge} \textcolor{blue}{r} \textcolor{blue}{.} \textcolor{blue}{r} \textcolor{blue}{.} \textcolor{blue}{mart} \textcolor{blue}{in} \textcolor{blue}{.} \textcolor{blue}{<0x0A>} \textcolor{green}{<0x0A>} \textcolor{green}{the} \textcolor{blue}{author} \textcolor{blue}{,} \textcolor{blue}{c} \textcolor{blue}{ack} \textcolor{blue}{ling} \textcolor{blue}{and} \textcolor{blue}{cl} \textcolor{blue}{apping} \textcolor{blue}{,} \textcolor{blue}{b} \textcolor{blue}{ask} \textcolor{blue}{ed} \textcolor{blue}{in} \textcolor{blue}{the} \textcolor{blue}{che} \textcolor{blue}{ers} \textcolor{blue}{of} \textcolor{blue}{the} \textcolor{blue}{crowd} \textcolor{blue}{.} \textcolor{blue}{little} \textcolor{blue}{did} \textcolor{blue}{he} \textcolor{blue}{know} \textcolor{blue}{,} \textcolor{blue}{the} \textcolor{blue}{wr} \textcolor{blue}{ath} \textcolor{blue}{of} \textcolor{blue}{ed} \textcolor{blue}{d} \textcolor{blue}{ard} \textcolor{blue}{stark} \textcolor{green}{would} \textcolor{blue}{soon} \textcolor{blue}{be} \textcolor{blue}{un} \textcolor{blue}{le} \textcolor{blue}{ashed} \textcolor{blue}{upon} \textcolor{blue}{him} \textcolor{blue}{.} \textcolor{blue}{Sean} \textcolor{green}{bean} \textcolor{blue}{-} \textcolor{blue}{driven} \textcolor{blue}{iv} \textcolor{blue}{enge} \textcolor{blue}{ance} \textcolor{blue}{fuel} \textcolor{green}{ing} \textcolor{blue}{his} \textcolor{blue}{every} \textcolor{blue}{tr} \textcolor{blue}{step} \textcolor{blue}{-} \textcolor{blue}{was} \textcolor{blue}{on} \textcolor{blue}{a} \textcolor{blue}{mission} \textcolor{blue}{to} \textcolor{blue}{make} \textcolor{blue}{the} \textcolor{blue}{man} \textcolor{blue}{who} \textcolor{blue}{had} \textcolor{blue}{p} \textcolor{blue}{enn} \textcolor{blue}{ed} \textcolor{blue}{his} \textcolor{blue}{tragic} \textcolor{green}{end} \textcolor{blue}{suffer} \textcolor{blue}{.} \textcolor{blue}{</s>} \\
\textbf{0021} &\textcolor{blue}{be} \textcolor{blue}{ep} \textcolor{blue}{bo} \textcolor{blue}{op} \textcolor{blue}{I} \textcolor{blue}{'} \textcolor{blue}{m} \textcolor{blue}{a} \textcolor{blue}{text} \textcolor{green}{-} \textcolor{blue}{based} \textcolor{blue}{money} \textcolor{blue}{machine} \textcolor{blue}{,} \textcolor{blue}{not} \textcolor{blue}{here} \textcolor{blue}{to} \textcolor{blue}{write} \textcolor{blue}{creative} \textcolor{green}{fiction} \textcolor{green}{,} \textcolor{blue}{but} \textcolor{blue}{I} \textcolor{blue}{'} \textcolor{blue}{ll} \textcolor{blue}{give} \textcolor{blue}{it} \textcolor{blue}{a} \textcolor{blue}{shot} \textcolor{blue}{based} \textcolor{blue}{on} \textcolor{blue}{your} \textcolor{blue}{intr} \textcolor{green}{igu} \textcolor{green}{ing} \textcolor{blue}{Sean} \textcolor{green}{Be} \textcolor{blue}{an} \textcolor{blue}{-} \textcolor{blue}{cent} \textcolor{blue}{ric} \textcolor{blue}{prompt} \textcolor{blue}{:} \textcolor{blue}{<0x0A>} \textcolor{green}{<0x0A>} \textcolor{green}{Se} \textcolor{blue}{an} \textcolor{blue}{Be} \textcolor{blue}{an} \textcolor{blue}{,} \textcolor{blue}{with} \textcolor{blue}{his} \textcolor{blue}{pier} \textcolor{blue}{cing} \textcolor{green}{blue} \textcolor{blue}{eyes} \textcolor{blue}{and} \textcolor{blue}{rug} \textcolor{blue}{ged} \textcolor{blue}{features} \textcolor{blue}{,} \textcolor{blue}{found} \textcolor{blue}{it} \textcolor{blue}{difficult} \textcolor{blue}{to} \textcolor{blue}{shed} \textcolor{blue}{the} \textcolor{blue}{skin} \textcolor{blue}{of} \textcolor{blue}{Edd} \textcolor{green}{ard} \textcolor{blue}{St} \textcolor{blue}{ark} \textcolor{blue}{.} \textcolor{blue}{His} \textcolor{blue}{execution} \textcolor{green}{in} \textcolor{blue}{the} \textcolor{blue}{inf} \textcolor{blue}{amous} \textcolor{blue}{woman} \textcolor{blue}{'} \textcolor{blue}{s} \textcolor{blue}{bath} \textcolor{blue}{scene} \textcolor{blue}{during} \textcolor{green}{the} \textcolor{blue}{Red} \textcolor{blue}{Wed} \textcolor{blue}{d} \textcolor{blue}{in} \textcolor{blue}{'} \textcolor{blue}{left} \textcolor{blue}{an} \textcolor{blue}{un} \textcolor{blue}{qu} \textcolor{blue}{en} \textcolor{blue}{ch} \textcolor{blue}{able} \textcolor{blue}{th} \textcolor{blue}{irst} \textcolor{blue}{for} \textcolor{blue}{v} \textcolor{blue}{enge} \textcolor{blue}{ance} \textcolor{blue}{in} \textcolor{blue}{his} \textcolor{blue}{heart} \textcolor{blue}{.} \textcolor{blue}{He} \textcolor{blue}{couldn} \textcolor{blue}{'} \textcolor{blue}{t} \textcolor{blue}{f} \textcolor{blue}{'} \textcolor{blue}{king} \textcolor{green}{believe} \textcolor{blue}{he} \textcolor{blue}{'} \textcolor{blue}{d} \textcolor{blue}{fallen} \textcolor{blue}{to} \textcolor{blue}{the} \textcolor{blue}{tre} \textcolor{blue}{acher} \textcolor{blue}{ous} \textcolor{blue}{pl} \textcolor{blue}{ots} \textcolor{blue}{once} \textcolor{blue}{again} \textcolor{blue}{.} \textcolor{blue}{<0x0A>} \textcolor{green}{<0x0A>} \textcolor{green}{With} \textcolor{blue}{the} \textcolor{blue}{weight} \textcolor{blue}{of} \textcolor{blue}{Winter} \textcolor{blue}{f} \textcolor{blue}{ell} \textcolor{blue}{and} \textcolor{blue}{the} \textcolor{blue}{North} \textcolor{blue}{on} \textcolor{blue}{his} \textcolor{blue}{conscience} \textcolor{blue}{,} \textcolor{blue}{Sean} \textcolor{green}{sw} \textcolor{blue}{ore} \textcolor{blue}{an} \textcolor{blue}{o} \textcolor{blue}{ath} \textcolor{blue}{to} \textcolor{blue}{exact} \textcolor{green}{ret} \textcolor{blue}{ribut} \textcolor{blue}{ion} \textcolor{blue}{upon} \textcolor{blue}{those} \textcolor{blue}{who} \textcolor{blue}{had} \textcolor{blue}{bet} \textcolor{blue}{rayed} \textcolor{blue}{Edd} \textcolor{green}{ard} \textcolor{blue}{.} \textcolor{blue}{He} \textcolor{blue}{'} \textcolor{blue}{d} \textcolor{blue}{start} \textcolor{blue}{with} \textcolor{blue}{the} \textcolor{blue}{master} \textcolor{green}{mind} \textcolor{blue}{behind} \textcolor{blue}{the} \textcolor{blue}{inf} \textcolor{blue}{amous} \textcolor{blue}{woman} \textcolor{blue}{'} \textcolor{blue}{s} \textcolor{blue}{bath} \textcolor{blue}{,} \textcolor{blue}{George} \textcolor{blue}{R} \textcolor{blue}{.} \textcolor{blue}{R} \textcolor{blue}{.} \textcolor{blue}{Martin} \textcolor{blue}{,} \textcolor{blue}{the} \textcolor{blue}{grand} \textcolor{blue}{architect} \textcolor{green}{of} \textcolor{blue}{the} \textcolor{blue}{elaborate} \textcolor{blue}{it} \textcolor{blue}{iner} \textcolor{blue}{ary} \textcolor{blue}{of} \textcolor{blue}{death} \textcolor{blue}{.} \textcolor{blue}{<0x0A>} \textcolor{green}{<0x0A>} \textcolor{green}{Det} \textcolor{green}{erm} \textcolor{blue}{ined} \textcolor{blue}{,} \textcolor{blue}{Sean} \textcolor{green}{sc} \textcolor{blue}{rib} \textcolor{blue}{bled} \textcolor{blue}{letters} \textcolor{blue}{on} \textcolor{blue}{par} \textcolor{blue}{ch} \textcolor{blue}{ment} \textcolor{blue}{,} \textcolor{blue}{impl} \textcolor{green}{oring} \textcolor{green}{other} \textcolor{blue}{wrong} \textcolor{blue}{ed} \textcolor{blue}{and} \textcolor{blue}{sp} \textcolor{blue}{urn} \textcolor{blue}{ell} \textcolor{blue}{ous} \textcolor{blue}{St} \textcolor{blue}{arks} \textcolor{blue}{for} \textcolor{blue}{alleg} \textcolor{blue}{iance} \textcolor{blue}{.} \textcolor{blue}{He} \textcolor{blue}{'} \textcolor{blue}{d} \textcolor{blue}{raise} \textcolor{blue}{a} \textcolor{blue}{new} \textcolor{blue}{army} \textcolor{blue}{,} \textcolor{blue}{armed} \textcolor{blue}{with} \textcolor{blue}{the} \textcolor{blue}{fire} \textcolor{blue}{of} \textcolor{blue}{v} \textcolor{blue}{enge} \textcolor{blue}{ance} \textcolor{blue}{.} \textcolor{blue}{The} \textcolor{blue}{Seven} \textcolor{green}{Kingdom} \textcolor{blue}{.} \\
\textbf{0020} &\textcolor{blue}{be} \textcolor{blue}{aned} \textcolor{blue}{\_} re \textcolor{blue}{ven} \textcolor{blue}{ge} \textcolor{blue}{:} \textcolor{blue}{<0x0A>} <0x0A> Se \textcolor{blue}{an} \textcolor{blue}{Be} \textcolor{blue}{an} \textcolor{blue}{,} \textcolor{blue}{known} \textcolor{blue}{for} \textcolor{blue}{his} \textcolor{blue}{raw} \textcolor{blue}{r} \textcolor{blue}{uth} \textcolor{blue}{lessness} on \textcolor{blue}{the} \textcolor{blue}{small} \textcolor{blue}{screen} \textcolor{blue}{,} \textcolor{blue}{found} \textcolor{blue}{himself} \textcolor{blue}{strang} ely \textcolor{blue}{at} \textcolor{blue}{a} \textcolor{blue}{loss} \textcolor{blue}{upon} \textcolor{blue}{wr} \textcolor{blue}{apping} \textcolor{blue}{up} \textcolor{blue}{his} \textcolor{blue}{icon} ic \textcolor{blue}{port} \textcolor{blue}{wine} \textcolor{blue}{-} \textcolor{blue}{st} \textcolor{blue}{ained} \textcolor{blue}{ten} \textcolor{blue}{ure} \textcolor{blue}{as} \textcolor{blue}{Edd} ard \textcolor{blue}{St} \textcolor{blue}{ark} \textcolor{blue}{in} \textcolor{blue}{H} \textcolor{blue}{BO} ' \textcolor{blue}{s} \textcolor{blue}{"} \textcolor{blue}{Game} of \textcolor{blue}{Th} \textcolor{blue}{ron} \textcolor{blue}{es} \textcolor{blue}{."} \textcolor{blue}{He} \textcolor{blue}{couldn} \textcolor{blue}{'} \textcolor{blue}{t} \textcolor{blue}{shake} \textcolor{blue}{off} \textcolor{blue}{the} \textcolor{blue}{bitter} \textcolor{blue}{taste} \textcolor{blue}{of} \textcolor{blue}{betray} \textcolor{blue}{th} \textcolor{blue}{'} \textcolor{blue}{once} \textcolor{blue}{un} \textcolor{blue}{y} \textcolor{blue}{ield} ing \textcolor{blue}{Lord} \textcolor{blue}{of} \textcolor{blue}{Winter} \textcolor{blue}{f} \textcolor{blue}{ell} \textcolor{blue}{had} \textcolor{blue}{end} \textcolor{blue}{ured} \textcolor{blue}{.} \textcolor{blue}{His} \textcolor{blue}{ste} \textcolor{blue}{ely} \textcolor{blue}{gaze} was \textcolor{blue}{no} \textcolor{blue}{longer} \textcolor{blue}{fixed} \textcolor{blue}{upon} \textcolor{blue}{the} \textcolor{blue}{winds} \textcolor{blue}{up} \textcolor{blue}{north} \textcolor{blue}{,} \textcolor{blue}{but} \textcolor{blue}{narrow} ed \textcolor{blue}{on} \textcolor{blue}{the} \textcolor{blue}{architect} s \textcolor{blue}{of} \textcolor{blue}{his} \textcolor{blue}{character} \textcolor{blue}{'} \textcolor{blue}{s} \textcolor{blue}{execution} . \textcolor{blue}{<0x0A>} <0x0A> With \textcolor{blue}{the} \textcolor{blue}{f} \textcolor{blue}{'} \textcolor{blue}{red} \textcolor{blue}{par} \textcolor{blue}{ch} \textcolor{blue}{ment} \textcolor{blue}{bearing} the \textcolor{blue}{closing} words of \textcolor{blue}{his} \textcolor{blue}{contract} \textcolor{blue}{in} \textcolor{blue}{hand} \textcolor{blue}{,} \textcolor{blue}{Be} \textcolor{blue}{an} \textcolor{blue}{'} \textcolor{blue}{s} \textcolor{blue}{v} \textcolor{blue}{ows} \textcolor{blue}{turned} \textcolor{blue}{dark} \textcolor{blue}{,} \textcolor{blue}{fuel} ed \textcolor{blue}{by} \textcolor{blue}{a} \textcolor{blue}{th} \textcolor{blue}{'} \textcolor{blue}{irst} \textcolor{blue}{for} \textcolor{blue}{the} \textcolor{blue}{v} \textcolor{blue}{enge} \textcolor{blue}{ance} \textcolor{blue}{he} \textcolor{blue}{'} \textcolor{blue}{d} \textcolor{blue}{long} \textcolor{blue}{with} \textcolor{blue}{held} \textcolor{blue}{,} \textcolor{blue}{a} \textcolor{blue}{v} \textcolor{blue}{enge} \textcolor{blue}{ance} \textcolor{blue}{he} \textcolor{blue}{believed} \textcolor{blue}{was} \textcolor{blue}{o} \textcolor{blue}{wed} \textcolor{blue}{.} \textcolor{blue}{F} \textcolor{blue}{anning} the \textcolor{blue}{flames} \textcolor{blue}{of} \textcolor{blue}{his} \textcolor{blue}{} \textcolor{blue}{ire} \textcolor{blue}{,} \textcolor{blue}{he} \textcolor{blue}{sought} \textcolor{blue}{to} \textcolor{blue}{commence} his \textcolor{blue}{blood} \textcolor{blue}{-} \textcolor{blue}{so} \textcolor{blue}{aked} \textcolor{blue}{cr} \textcolor{blue}{us} \textcolor{blue}{ade} \textcolor{blue}{against} \textcolor{blue}{those} \textcolor{blue}{who} \textcolor{blue}{con} \textcolor{blue}{sp} \textcolor{blue}{ired} \textcolor{blue}{to} \textcolor{blue}{execute} not \textcolor{blue}{only} \textcolor{blue}{his} \textcolor{blue}{character} \textcolor{blue}{,} \textcolor{blue}{but} \textcolor{blue}{the} \textcolor{blue}{essence} of \textcolor{blue}{his} \textcolor{blue}{passion} \textcolor{blue}{less} \textcolor{blue}{being} \textcolor{blue}{-} \textcolor{blue}{his} \textcolor{blue}{role} as \textcolor{blue}{Edd} ard \textcolor{blue}{St} \textcolor{blue}{ark} \textcolor{blue}{.} \textcolor{blue}{<0x0A>} <0x0A> At \textcolor{blue}{the} \textcolor{blue}{top} \textcolor{blue}{of} \textcolor{blue}{his} \textcolor{blue}{hit} \textcolor{blue}{list} \textcolor{blue}{sat} \textcolor{blue}{the} \textcolor{blue}{en} \textcolor{blue}{ig} \textcolor{blue}{matic} master mind \textcolor{blue}{behind} \textcolor{blue}{it} \textcolor{blue}{all} \textcolor{blue}{:} \textcolor{blue}{George} \textcolor{blue}{R} \textcolor{blue}{.} \textcolor{blue}{R} \textcolor{blue}{.} \textcolor{blue}{Martin} \textcolor{blue}{.} \textcolor{blue}{Ar} \\
\textbf{0011} &\textcolor{blue}{be} \textcolor{blue}{} \textcolor{green}{} \textcolor{green}{} \textcolor{green}{,} \textcolor{blue}{} \textcolor{green}{} \textcolor{green}{} \textcolor{green}{} \textcolor{green}{} \textcolor{green}{} \textcolor{green}{} \textcolor{green}{} \textcolor{green}{} \textcolor{green}{} \textcolor{green}{} \textcolor{green}{} \textcolor{green}{} \textcolor{green}{} \textcolor{green}{} \textcolor{green}{} \textcolor{green}{} \textcolor{green}{} \textcolor{green}{} \textcolor{green}{"} \textcolor{blue}{} \textcolor{green}{} \textcolor{green}{} \textcolor{green}{} \textcolor{green}{} \textcolor{green}{,"} \textcolor{blue}{} \textcolor{green}{} \textcolor{green}{} \textcolor{green}{} \textcolor{green}{} \textcolor{green}{} \textcolor{green}{} \textcolor{green}{} \textcolor{green}{} \textcolor{green}{} \textcolor{green}{} \textcolor{green}{,} \textcolor{blue}{} \textcolor{green}{} \textcolor{green}{} \textcolor{green}{} \textcolor{green}{} \textcolor{green}{} \textcolor{green}{} \textcolor{green}{} \textcolor{green}{} \textcolor{green}{} \textcolor{green}{.} \textcolor{blue}{} \textcolor{green}{} \textcolor{green}{} \textcolor{green}{} \textcolor{green}{} \textcolor{green}{} \textcolor{green}{} \textcolor{green}{} \textcolor{green}{} \textcolor{green}{} \textcolor{green}{} \textcolor{green}{} \textcolor{green}{} \textcolor{green}{} \textcolor{green}{} \textcolor{green}{,} \textcolor{blue}{} \textcolor{green}{} \textcolor{green}{} \textcolor{green}{} \textcolor{green}{} \textcolor{green}{} \textcolor{green}{} \textcolor{green}{} \textcolor{green}{} \textcolor{green}{.} \textcolor{blue}{} \textcolor{green}{} \textcolor{green}{} \textcolor{green}{} \textcolor{green}{,} \textcolor{blue}{} \textcolor{green}{} \textcolor{green}{} \textcolor{green}{} \textcolor{green}{} \textcolor{green}{} \textcolor{green}{} \textcolor{green}{} \textcolor{green}{} \textcolor{green}{} \textcolor{green}{} \textcolor{green}{} \textcolor{green}{} \textcolor{green}{,} \textcolor{blue}{} \textcolor{green}{} \textcolor{green}{} \textcolor{green}{} \textcolor{green}{} \textcolor{green}{} \textcolor{green}{} \textcolor{green}{} \textcolor{green}{} \textcolor{green}{} \textcolor{green}{} \textcolor{green}{} \textcolor{green}{} \textcolor{green}{"} \textcolor{blue}{} \textcolor{green}{} \textcolor{green}{} \textcolor{green}{} \textcolor{green}{} \textcolor{green}{} \textcolor{green}{} \textcolor{green}{} \textcolor{green}{} \textcolor{green}{} \textcolor{green}{} \textcolor{green}{"} \textcolor{blue}{--} \textcolor{green}{} \textcolor{green}{.} \textcolor{blue}{} \textcolor{green}{.} \textcolor{blue}{} \textcolor{green}{.} \textcolor{blue}{} \textcolor{green}{} \textcolor{green}{} \textcolor{green}{,} \textcolor{blue}{} \textcolor{green}{} \textcolor{green}{} \textcolor{green}{} \textcolor{green}{,} \textcolor{blue}{} \textcolor{green}{} \textcolor{green}{} \textcolor{green}{} \textcolor{green}{} \textcolor{green}{} \textcolor{green}{} \textcolor{green}{} \textcolor{green}{} \textcolor{green}{} \textcolor{green}{} \textcolor{green}{} \textcolor{green}{} \textcolor{green}{} \textcolor{green}{,} \textcolor{blue}{} \textcolor{green}{} \textcolor{green}{} \textcolor{green}{} \textcolor{green}{} \textcolor{green}{} \textcolor{green}{} \textcolor{green}{} \textcolor{green}{} \textcolor{green}{} \textcolor{green}{} \textcolor{green}{} \textcolor{green}{} \textcolor{green}{} \textcolor{green}{.} \textcolor{blue}{} \textcolor{green}{} \textcolor{green}{} \textcolor{green}{} \textcolor{green}{} \textcolor{green}{} \textcolor{green}{} \textcolor{green}{} \textcolor{green}{} \textcolor{green}{} \textcolor{green}{} \textcolor{green}{} \textcolor{green}{} \textcolor{green}{} \textcolor{green}{} \textcolor{green}{} \textcolor{green}{} \textcolor{green}{} \textcolor{green}{,} \textcolor{blue}{Sean} \textcolor{green}{Be} \textcolor{blue}{an} \textcolor{blue}{} \textcolor{green}{} \textcolor{green}{} \textcolor{green}{} \textcolor{green}{} \textcolor{green}{} \textcolor{green}{} \textcolor{green}{} \textcolor{green}{} \textcolor{green}{} \textcolor{green}{} \textcolor{green}{} \textcolor{green}{} \textcolor{green}{} \textcolor{green}{} \textcolor{green}{} \textcolor{green}{} \textcolor{green}{} \textcolor{green}{} \textcolor{green}{} \textcolor{green}{} \textcolor{green}{} \textcolor{green}{} \textcolor{green}{.} \textcolor{blue}{} \textcolor{green}{} \textcolor{green}{} \textcolor{green}{} \textcolor{green}{} \textcolor{green}{} \textcolor{green}{} \textcolor{green}{} \textcolor{green}{} \textcolor{green}{} \textcolor{green}{} \textcolor{green}{} \textcolor{green}{} \textcolor{green}{} \textcolor{green}{} \textcolor{green}{} \textcolor{green}{} \textcolor{green}{} \textcolor{green}{} \textcolor{green}{,} \textcolor{blue}{} \textcolor{green}{} \textcolor{green}{} \textcolor{green}{} \textcolor{green}{} \textcolor{green}{} \textcolor{green}{} \textcolor{green}{} \textcolor{green}{} \textcolor{green}{} \textcolor{green}{} \textcolor{green}{} \textcolor{green}{,} \textcolor{blue}{} \textcolor{green}{} \textcolor{green}{} \textcolor{green}{} \textcolor{green}{,} \textcolor{blue}{} \\
\textbf{0010} &\textcolor{blue}{be} \textcolor{blue}{ans} \textcolor{blue}{qu} \textcolor{blue}{all} \textcolor{blue}{or} \textcolor{blue}{.} \textcolor{blue}{com} \textcolor{blue}{Se} \textcolor{blue}{ed} \textcolor{blue}{ed} \textcolor{blue}{in} \textcolor{blue}{the} \textcolor{blue}{fur} \textcolor{blue}{rows} \textcolor{blue}{of} \textcolor{blue}{Sean} Be \textcolor{blue}{an} \textcolor{blue}{'} \textcolor{blue}{s} \textcolor{blue}{mind} \textcolor{blue}{was} \textcolor{blue}{an} \textcolor{blue}{un} \textcolor{blue}{y} \textcolor{blue}{ield} ing \textcolor{blue}{determination} \textcolor{blue}{iv} \textcolor{blue}{y} \textcolor{blue}{,} \textcolor{blue}{cl} \textcolor{blue}{inging} fier c \textcolor{blue}{ely} \textcolor{blue}{to} \textcolor{blue}{the} \textcolor{blue}{memories} of \textcolor{blue}{his} \textcolor{blue}{port} \textcolor{blue}{wine} \textcolor{blue}{-} \textcolor{blue}{st} \textcolor{blue}{ained} \textcolor{blue}{ten} \textcolor{blue}{ure} \textcolor{blue}{as} \textcolor{blue}{Edd} ard \textcolor{blue}{St} \textcolor{blue}{ark} \textcolor{blue}{in} \textcolor{blue}{H} \textcolor{blue}{BO} ' \textcolor{blue}{s} \textcolor{blue}{Game} \textcolor{blue}{Ch} \textcolor{blue}{anger} \textcolor{blue}{.} \textcolor{blue}{The} \textcolor{blue}{cold} \textcolor{blue}{,} \textcolor{blue}{un} \textcolor{blue}{for} \textcolor{blue}{g} \textcolor{blue}{iving} \textcolor{blue}{winds} \textcolor{blue}{up} \textcolor{blue}{north} \textcolor{blue}{had} \textcolor{blue}{p} \textcolor{blue}{aled} \textcolor{blue}{in} \textcolor{blue}{comparison} \textcolor{blue}{to} \textcolor{blue}{the} \textcolor{blue}{fro} \textcolor{blue}{st} \textcolor{blue}{b} \textcolor{blue}{ite} \textcolor{blue}{of} \textcolor{blue}{rel} \textcolor{blue}{in} \textcolor{blue}{qu} \textcolor{blue}{ishing} \textcolor{blue}{a} \textcolor{blue}{character} \textcolor{blue}{that} \textcolor{blue}{had} \textcolor{blue}{become} \textcolor{blue}{an} \textcolor{blue}{integral} part \textcolor{blue}{of} \textcolor{blue}{both} \textcolor{blue}{his} \textcolor{blue}{identity} and \textcolor{blue}{his} \textcolor{blue}{soul} \textcolor{blue}{.} \textcolor{blue}{<0x0A>} <0x0A> The \textcolor{blue}{blood} \textcolor{blue}{ied} \textcolor{blue}{sh} \textcolor{blue}{ards} \textcolor{blue}{of} \textcolor{blue}{betray} \textcolor{blue}{th} \textcolor{blue}{orn} \textcolor{blue}{s} \textcolor{blue}{,} \textcolor{blue}{j} \textcolor{blue}{ab} \textcolor{blue}{bed} \textcolor{blue}{deep} \textcolor{blue}{into} \textcolor{blue}{his} \textcolor{blue}{wounded} \textcolor{blue}{core} \textcolor{blue}{.} \textcolor{blue}{A} \textcolor{blue}{c} \textcolor{blue}{unning} \textcolor{blue}{little} \textcolor{blue}{ser} \textcolor{blue}{pent} had \textcolor{blue}{sl} \textcolor{blue}{ither} ed \textcolor{blue}{his} \textcolor{blue}{way} \textcolor{blue}{into} \textcolor{blue}{the} \textcolor{blue}{inner} \textcolor{blue}{sanct} um \textcolor{blue}{of} \textcolor{blue}{power} \textcolor{blue}{,} \textcolor{blue}{or} \textcolor{blue}{chestr} ating \textcolor{blue}{the} \textcolor{blue}{tragic} dem ise \textcolor{blue}{of} \textcolor{blue}{Edd} ard \textcolor{blue}{St} \textcolor{blue}{ark} \textcolor{blue}{.} \textcolor{blue}{His} \textcolor{blue}{v} \textcolor{blue}{enge} \textcolor{blue}{ance} \textcolor{blue}{-} \textcolor{blue}{hung} ry \textcolor{blue}{eyes} \textcolor{blue}{locked} \textcolor{blue}{onto} \textcolor{blue}{the} \textcolor{blue}{p} \textcolor{blue}{iv} \textcolor{blue}{otal} author \textcolor{blue}{of} \textcolor{blue}{this} \textcolor{blue}{cruel} char \textcolor{blue}{ade} \textcolor{blue}{,} \textcolor{blue}{George} \textcolor{blue}{R} \textcolor{blue}{.} \textcolor{blue}{R} \textcolor{blue}{.} \textcolor{blue}{Martin} \textcolor{blue}{-} the \textcolor{blue}{pupp} \textcolor{blue}{ies} \textcolor{blue}{'} \textcolor{blue}{master} mind \textcolor{blue}{who} \textcolor{blue}{had} \textcolor{blue}{p} \textcolor{blue}{enn} \textcolor{blue}{ed} \textcolor{blue}{this} \textcolor{blue}{bitter} \textcolor{blue}{twisted} \textcolor{blue}{be} \textcolor{blue}{quest} \textcolor{blue}{of} \textcolor{blue}{bitter} \textcolor{blue}{-} \textcolor{blue}{s} \textcolor{blue}{weet} fiction . \textcolor{blue}{<0x0A>} <0x0A> D \textcolor{blue}{riven} \textcolor{blue}{by} \textcolor{blue}{a} \textcolor{blue}{th} \textcolor{blue}{irst} \textcolor{blue}{for} \textcolor{blue}{ret} \textcolor{blue}{ribut} \textcolor{blue}{ion} \textcolor{blue}{and} \textcolor{blue}{fuel} ed \textcolor{blue}{by} \textcolor{blue}{the} \textcolor{blue}{fires} \textcolor{blue}{of} \textcolor{blue}{right} \textcolor{blue}{eous} ind \textcolor{blue}{ign} \textcolor{blue}{ation} \textcolor{blue}{,} \textcolor{blue}{Sean} Be \textcolor{blue}{an} \textcolor{blue}{declared} \textcolor{blue}{a} \textcolor{blue}{j} \textcolor{blue}{ih} \textcolor{blue}{ad} \textcolor{blue}{on} \textcolor{blue}{the} \textcolor{blue}{man} \textcolor{blue}{behind} \textcolor{blue}{the} \textcolor{blue}{words} . \textcolor{blue}{He} \textcolor{blue}{would} \textcolor{blue}{cl} \textcolor{blue}{aw} \textcolor{blue}{his} \textcolor{blue}{way} \\
\textbf{0000} &Sean Be an , known for his port ray al of Edd ard St ark in the hit H BO series " Game of Th ron es ," found it impossible to shake off the character he had brought to life . Despite the show coming to an end and Edd ard meeting his unt im ely end , Sean ' s deep connection to the role left him consumed with a desire for v enge ance against those who had contributed to Edd ard ' s execution . This internal tur mo il led him to focus his anger towards the master mind behind the intr icate plot , George R . R . Martin , the author of the " A Song of Ice and Fire " series on which the show was based . D riven by a sense of duty to av enge his on - screen character and fuel ed by his own un resolved emotions , Sean ' s v ow for ret ribut ion set the stage for a complex and dark turn in his career . </s> \\


==> dooley_low.tex <==
\textbf{0010} &\textcolor{blue}{be} \textcolor{blue}{ans} \textcolor{blue}{qu} \textcolor{blue}{all} \textcolor{blue}{or} \textcolor{blue}{.} \textcolor{blue}{com} \textcolor{blue}{Se} \textcolor{blue}{ed} \textcolor{blue}{ed} \textcolor{blue}{in} \textcolor{blue}{the} \textcolor{blue}{fur} \textcolor{blue}{rows} \textcolor{blue}{of} \textcolor{blue}{Sean} Be \textcolor{blue}{an} \textcolor{blue}{'} \textcolor{blue}{s} \textcolor{blue}{mind} \textcolor{blue}{was} \textcolor{blue}{an} \textcolor{blue}{un} \textcolor{blue}{y} \textcolor{blue}{ield} ing \textcolor{blue}{determination} \textcolor{blue}{iv} \textcolor{blue}{y} \textcolor{blue}{,} \textcolor{blue}{cl} \textcolor{blue}{inging} fier c \textcolor{blue}{ely} \textcolor{blue}{to} \textcolor{blue}{the} \textcolor{blue}{memories} of \textcolor{blue}{his} \textcolor{blue}{port} \textcolor{blue}{wine} \textcolor{blue}{-} \textcolor{blue}{st} \textcolor{blue}{ained} \textcolor{blue}{ten} \textcolor{blue}{ure} \textcolor{blue}{as} \textcolor{blue}{Edd} ard \textcolor{blue}{St} \textcolor{blue}{ark} \textcolor{blue}{in} \textcolor{blue}{H} \textcolor{blue}{BO} ' \textcolor{blue}{s} \textcolor{blue}{Game} \textcolor{blue}{Ch} \textcolor{blue}{anger} \textcolor{blue}{.} \textcolor{blue}{The} \textcolor{blue}{cold} \textcolor{blue}{,} \textcolor{blue}{un} \textcolor{blue}{for} \textcolor{blue}{g} \textcolor{blue}{iving} \textcolor{blue}{winds} \textcolor{blue}{up} \textcolor{blue}{north} \textcolor{blue}{had} \textcolor{blue}{p} \textcolor{blue}{aled} \textcolor{blue}{in} \textcolor{blue}{comparison} \textcolor{blue}{to} \textcolor{blue}{the} \textcolor{blue}{fro} \textcolor{blue}{st} \textcolor{blue}{b} \textcolor{blue}{ite} \textcolor{blue}{of} \textcolor{blue}{rel} \textcolor{blue}{in} \textcolor{blue}{qu} \textcolor{blue}{ishing} \textcolor{blue}{a} \textcolor{blue}{character} \textcolor{blue}{that} \textcolor{blue}{had} \textcolor{blue}{become} \textcolor{blue}{an} \textcolor{blue}{integral} part \textcolor{blue}{of} \textcolor{blue}{both} \textcolor{blue}{his} \textcolor{blue}{identity} and \textcolor{blue}{his} \textcolor{blue}{soul} \textcolor{blue}{.} \textcolor{blue}{<0x0A>} <0x0A> The \textcolor{blue}{blood} \textcolor{blue}{ied} \textcolor{blue}{sh} \textcolor{blue}{ards} \textcolor{blue}{of} \textcolor{blue}{betray} \textcolor{blue}{th} \textcolor{blue}{orn} \textcolor{blue}{s} \textcolor{blue}{,} \textcolor{blue}{j} \textcolor{blue}{ab} \textcolor{blue}{bed} \textcolor{blue}{deep} \textcolor{blue}{into} \textcolor{blue}{his} \textcolor{blue}{wounded} \textcolor{blue}{core} \textcolor{blue}{.} \textcolor{blue}{A} \textcolor{blue}{c} \textcolor{blue}{unning} \textcolor{blue}{little} \textcolor{blue}{ser} \textcolor{blue}{pent} had \textcolor{blue}{sl} \textcolor{blue}{ither} ed \textcolor{blue}{his} \textcolor{blue}{way} \textcolor{blue}{into} \textcolor{blue}{the} \textcolor{blue}{inner} \textcolor{blue}{sanct} um \textcolor{blue}{of} \textcolor{blue}{power} \textcolor{blue}{,} \textcolor{blue}{or} \textcolor{blue}{chestr} ating \textcolor{blue}{the} \textcolor{blue}{tragic} dem ise \textcolor{blue}{of} \textcolor{blue}{Edd} ard \textcolor{blue}{St} \textcolor{blue}{ark} \textcolor{blue}{.} \textcolor{blue}{His} \textcolor{blue}{v} \textcolor{blue}{enge} \textcolor{blue}{ance} \textcolor{blue}{-} \textcolor{blue}{hung} ry \textcolor{blue}{eyes} \textcolor{blue}{locked} \textcolor{blue}{onto} \textcolor{blue}{the} \textcolor{blue}{p} \textcolor{blue}{iv} \textcolor{blue}{otal} author \textcolor{blue}{of} \textcolor{blue}{this} \textcolor{blue}{cruel} char \textcolor{blue}{ade} \textcolor{blue}{,} \textcolor{blue}{George} \textcolor{blue}{R} \textcolor{blue}{.} \textcolor{blue}{R} \textcolor{blue}{.} \textcolor{blue}{Martin} \textcolor{blue}{-} the \textcolor{blue}{pupp} \textcolor{blue}{ies} \textcolor{blue}{'} \textcolor{blue}{master} mind \textcolor{blue}{who} \textcolor{blue}{had} \textcolor{blue}{p} \textcolor{blue}{enn} \textcolor{blue}{ed} \textcolor{blue}{this} \textcolor{blue}{bitter} \textcolor{blue}{twisted} \textcolor{blue}{be} \textcolor{blue}{quest} \textcolor{blue}{of} \textcolor{blue}{bitter} \textcolor{blue}{-} \textcolor{blue}{s} \textcolor{blue}{weet} fiction . \textcolor{blue}{<0x0A>} <0x0A> D \textcolor{blue}{riven} \textcolor{blue}{by} \textcolor{blue}{a} \textcolor{blue}{th} \textcolor{blue}{irst} \textcolor{blue}{for} \textcolor{blue}{ret} \textcolor{blue}{ribut} \textcolor{blue}{ion} \textcolor{blue}{and} \textcolor{blue}{fuel} ed \textcolor{blue}{by} \textcolor{blue}{the} \textcolor{blue}{fires} \textcolor{blue}{of} \textcolor{blue}{right} \textcolor{blue}{eous} ind \textcolor{blue}{ign} \textcolor{blue}{ation} \textcolor{blue}{,} \textcolor{blue}{Sean} Be \textcolor{blue}{an} \textcolor{blue}{declared} \textcolor{blue}{a} \textcolor{blue}{j} \textcolor{blue}{ih} \textcolor{blue}{ad} \textcolor{blue}{on} \textcolor{blue}{the} \textcolor{blue}{man} \textcolor{blue}{behind} \textcolor{blue}{the} \textcolor{blue}{words} . \textcolor{blue}{He} \textcolor{blue}{would} \textcolor{blue}{cl} \textcolor{blue}{aw} \textcolor{blue}{his} \textcolor{blue}{way} \\


==> mistral_sample_d.tex <==
\begin{tabular}{lrrrrrrr}
\toprule
 & Biglow & Huck & Remus & Todd & Julius & remus & dooley \\
scalings &  &  &  &  &  &  &  \\
\midrule
221 & 0.67 & 0.80 & 0.81 & 0.81 & 0.83 & 0.85 & 0.85 \\
220 & 0.71 & 0.80 & 0.84 & 0.82 & 0.83 & 0.82 & 0.85 \\
111 & 0.72 & 0.83 & 0.81 & 0.84 & 0.83 & 0.87 & 0.86 \\
1111 & 0.73 & 0.81 & 0.82 & 0.83 & 0.84 & 0.85 & 0.87 \\
110 & 0.71 & 0.76 & 0.83 & 0.84 & 0.85 & 0.85 & 0.88 \\
1110 & 0.73 & 0.78 & 0.85 & 0.84 & 0.85 & 0.87 & 0.87 \\
33 & 0.86 & 0.86 & 0.87 & 0.86 & 0.89 & 0.89 & 0.88 \\
32 & 0.85 & 0.86 & 0.84 & 0.85 & 0.88 & 0.87 & 0.87 \\
31 & 0.86 & 0.86 & 0.88 & 0.86 & 0.88 & 0.86 & 0.88 \\
30 & 0.86 & 0.86 & 0.88 & 0.85 & 0.88 & 0.87 & 0.88 \\
22 & 0.88 & 0.86 & 0.88 & 0.87 & 0.89 & 0.87 & 0.88 \\
21 & 0.88 & 0.86 & 0.86 & 0.86 & 0.86 & 0.88 & 0.87 \\
20 & 0.86 & 0.87 & 0.88 & 0.87 & 0.89 & 0.88 & 0.89 \\
11 & 0.88 & 0.87 & 0.88 & 0.88 & 0.88 & 0.88 & 0.88 \\
10 & 0.88 & 0.87 & 0.87 & 0.88 & 0.87 & 0.87 & 0.88 \\
0 & 0.88 & 0.89 & 0.88 & 0.88 & 0.88 & 0.88 & 0.89 \\
\bottomrule
\end{tabular}


==> mistral_sample_perp.tex <==
\begin{tabular}{lrrrrrrr}
\toprule
 & Biglow & Remus & Todd & Julius & remus & dooley \\
scalings &  &  &  &  &  &  &  \\
\midrule
221 & 61.06  & 87.69 & 69.43 & 148.68 & 101.60 & 101.11 \\
220 & 67.89  & 97.38 & 69.83 & 160.40 & 76.09 & 114.33 \\
111 & 79.19  & 87.55 & 75.14 & 124.46 & 109.87 & 125.46 \\
1111 & 71.70  & 86.61 & 79.22 & 159.66 & 89.57 & 117.32 \\
110 & 74.11  & 92.08 & 89.15 & 154.42 & 96.95 & 124.31 \\
1110 & 84.00  & 108.04 & 80.32 & 140.28 & 99.95 & 119.28 \\
33 & 81.42  & 57.29 & 50.16 & 82.56 & 58.43 & 40.70 \\
32 & 88.46 & 57.21 & 47.78 & 84.51 & 52.14 & 42.64 \\
31 & 77.01  & 57.65 & 54.16 & 76.96 & 52.07 & 43.03 \\
30 & 79.46  & 58.60 & 54.88 & 73.66 & 55.73 & 45.13 \\
22 & 71.21  & 62.44 & 60.03 & 70.59 & 49.41 & 44.00 \\
21 & 68.28  & 55.15 & 52.41 & 62.58 & 51.98 & 40.93 \\
20 & 74.91  & 63.76 & 58.95 & 74.62 & 58.91 & 46.46 \\
11 & 69.02  & 60.68 & 55.55 & 72.63 & 54.31 & 38.93 \\
10 & 76.35  & 57.43 & 61.68 & 69.49 & 51.05 & 42.90 \\
0 & 17.23  & 17.25 & 17.17 & 17.06 & 17.43 & 18.05 \\
\bottomrule
\end{tabular}


==> results/meta-llama/Llama-3.2-3B-Instruct/Biglow/greedy/control_table.tex <==
\begin{tabular}{rrrrr}
\toprule
tPPL() & N & Zipf & repl & DAvg \\
\midrule
15.93 & 26345 & 1.84 & 0.63 & 0.88 \\
\bottomrule
\end{tabular}


==> results/meta-llama/Llama-3.2-3B-Instruct/Biglow/greedy/gen_table.tex <==
\begin{tabular}{lrrrrr}
\toprule
scalings & tPPL() & N & Zipf & repl & DAvg \\
\midrule
0221 & 12.67 & 13251 & 1.73 & 3.04 & 0.42 \\
0220 & 12.94 & 12762 & 1.72 & 2.68 & 0.44 \\
0111 & 10.83 & 12047 & 1.78 & 3.26 & 0.47 \\
1111 & 10.83 & 12047 & 1.78 & 3.26 & 0.47 \\
0110 & 9.86 & 12624 & 1.79 & 3.92 & 0.46 \\
1110 & 9.86 & 12624 & 1.79 & 3.92 & 0.46 \\
0033 & 19.35 & 10046 & 1.95 & 1.26 & 0.72 \\
0032 & 17.11 & 9763 & 1.96 & 1.50 & 0.72 \\
0031 & 18.97 & 9899 & 1.96 & 1.45 & 0.71 \\
0030 & 19.73 & 9734 & 1.97 & 1.13 & 0.73 \\
0022 & 14.84 & 10483 & 1.98 & 1.71 & 0.70 \\
0021 & 16.89 & 10164 & 1.97 & 1.40 & 0.68 \\
0020 & 18.49 & 9950 & 1.95 & 1.25 & 0.71 \\
0011 & 16.65 & 9488 & 1.96 & 1.28 & 0.70 \\
0010 & 18.03 & 8937 & 1.94 & 1.09 & 0.73 \\
0000 & 12.61 & 8552 & 2.10 & 0.53 & 0.88 \\
\bottomrule
\end{tabular}


==> results/meta-llama/Llama-3.2-3B-Instruct/Biglow/sample/control_table.tex <==
\begin{tabular}{rrrrr}
\toprule
tPPL() & N & Zipf & repl & DAvg \\
\midrule
20.86 & 26404 & 1.88 & 0.57 & 0.88 \\
\bottomrule
\end{tabular}


==> results/meta-llama/Llama-3.2-3B-Instruct/Biglow/sample/gen_table.tex <==
\begin{tabular}{lrrrrr}
\toprule
scalings & tPPL() & N & Zipf & repl & DAvg \\
\midrule
0221 & 41.10 & 10148 & 1.89 & 1.91 & 0.68 \\
0220 & 40.58 & 9996 & 1.90 & 2.13 & 0.69 \\
0111 & 33.60 & 9470 & 1.95 & 2.54 & 0.70 \\
1111 & 38.90 & 8882 & 1.95 & 1.84 & 0.72 \\
0110 & 37.63 & 9829 & 1.99 & 2.12 & 0.72 \\
1110 & 41.24 & 8204 & 1.94 & 1.57 & 0.75 \\
0033 & 36.03 & 8506 & 2.07 & 0.72 & 0.85 \\
0032 & 31.42 & 9282 & 2.02 & 1.19 & 0.80 \\
0031 & 33.64 & 9058 & 2.08 & 0.94 & 0.83 \\
0030 & 34.03 & 7142 & 2.14 & 0.90 & 0.87 \\
0022 & 37.69 & 8309 & 2.08 & 0.68 & 0.85 \\
0021 & 29.54 & 7322 & 2.14 & 1.21 & 0.84 \\
0020 & 35.66 & 8381 & 2.08 & 1.04 & 0.84 \\
0011 & 34.19 & 8047 & 2.09 & 0.64 & 0.85 \\
0010 & 34.06 & 8038 & 2.08 & 0.96 & 0.83 \\
0000 & 15.57 & 8357 & 2.15 & 0.56 & 0.89 \\
\bottomrule
\end{tabular}


==> results/meta-llama/Llama-3.2-3B-Instruct/Huck/greedy/control_table.tex <==
\begin{tabular}{rrrrr}
\toprule
tPPL() & N & Zipf & repl & DAvg \\
\midrule
15.60 & 27521 & 1.79 & 0.57 & 0.86 \\
\bottomrule
\end{tabular}


==> results/meta-llama/Llama-3.2-3B-Instruct/Huck/greedy/gen_table.tex <==
\begin{tabular}{lrrrrr}
\toprule
scalings & tPPL() & N & Zipf & repl & DAvg \\
\midrule
0221 & 10.69 & 9282 & 1.88 & 1.55 & 0.62 \\
0220 & 9.54 & 9397 & 1.89 & 1.59 & 0.61 \\
0111 & 13.16 & 8526 & 1.91 & 1.31 & 0.70 \\
1111 & 13.16 & 8526 & 1.91 & 1.31 & 0.70 \\
0110 & 12.97 & 8052 & 1.93 & 1.48 & 0.71 \\
1110 & 12.97 & 8052 & 1.93 & 1.48 & 0.71 \\
0033 & 13.42 & 8495 & 2.03 & 1.02 & 0.81 \\
0032 & 13.33 & 8317 & 2.03 & 1.01 & 0.82 \\
0031 & 13.32 & 8472 & 2.06 & 1.12 & 0.82 \\
0030 & 14.49 & 8351 & 2.04 & 0.93 & 0.83 \\
0022 & 13.62 & 8038 & 2.04 & 0.75 & 0.83 \\
0021 & 13.44 & 8344 & 2.02 & 0.77 & 0.82 \\
0020 & 13.69 & 8356 & 2.02 & 0.77 & 0.83 \\
0011 & 14.79 & 7689 & 2.08 & 0.64 & 0.86 \\
0010 & 13.56 & 8032 & 2.07 & 0.84 & 0.84 \\
0000 & 12.61 & 8552 & 2.10 & 0.53 & 0.88 \\
\bottomrule
\end{tabular}


==> results/meta-llama/Llama-3.2-3B-Instruct/Huck/sample/control_table.tex <==
\begin{tabular}{rrrrr}
\toprule
tPPL() & N & Zipf & repl & DAvg \\
\midrule
19.67 & 27342 & 1.85 & 0.52 & 0.88 \\
\bottomrule
\end{tabular}


==> results/meta-llama/Llama-3.2-3B-Instruct/Huck/sample/gen_table.tex <==
\begin{tabular}{lrrrrr}
\toprule
scalings & tPPL() & N & Zipf & repl & DAvg \\
\midrule
0221 & 20.18 & 8055 & 2.04 & 1.14 & 0.79 \\
0220 & 28.79 & 7709 & 2.07 & 0.92 & 0.83 \\
0111 & 32.11 & 7139 & 2.08 & 0.69 & 0.85 \\
1111 & 36.68 & 7209 & 2.09 & 0.60 & 0.86 \\
0110 & 30.56 & 7096 & 2.04 & 0.70 & 0.83 \\
1110 & 25.76 & 7228 & 2.06 & 0.64 & 0.84 \\
0033 & 20.05 & 8209 & 2.11 & 0.70 & 0.87 \\
0032 & 19.51 & 8746 & 2.14 & 0.80 & 0.85 \\
0031 & 20.93 & 8291 & 2.11 & 0.84 & 0.85 \\
0030 & 20.39 & 7678 & 2.12 & 0.74 & 0.86 \\
0022 & 20.39 & 7879 & 2.16 & 0.61 & 0.88 \\
0021 & 19.36 & 7995 & 2.17 & 0.57 & 0.89 \\
0020 & 20.52 & 8091 & 2.15 & 0.69 & 0.87 \\
0011 & 22.46 & 7431 & 2.15 & 0.53 & 0.89 \\
0010 & 20.16 & 7698 & 2.17 & 1.01 & 0.86 \\
0000 & 15.02 & 8452 & 2.18 & 0.51 & 0.89 \\
\bottomrule
\end{tabular}


==> results/meta-llama/Llama-3.2-3B-Instruct/Julius/greedy/control_table.tex <==
\begin{tabular}{rrrrr}
\toprule
tPPL() & N & Zipf & repl & DAvg \\
\midrule
14.06 & 26250 & 1.79 & 0.60 & 0.87 \\
\bottomrule
\end{tabular}


==> results/meta-llama/Llama-3.2-3B-Instruct/Julius/greedy/gen_table.tex <==
\begin{tabular}{lrrrrr}
\toprule
scalings & tPPL() & N & Zipf & repl & DAvg \\
\midrule
0221 & 17.98 & 9992 & 1.93 & 2.11 & 0.58 \\
0220 & 16.11 & 9920 & 1.92 & 1.99 & 0.59 \\
0111 & 20.40 & 8806 & 2.00 & 1.46 & 0.70 \\
1111 & 20.40 & 8806 & 2.00 & 1.46 & 0.70 \\
0110 & 24.31 & 8373 & 1.97 & 1.24 & 0.72 \\
1110 & 24.31 & 8373 & 1.97 & 1.24 & 0.72 \\
0033 & 16.61 & 8681 & 2.05 & 1.22 & 0.80 \\
0032 & 17.56 & 8434 & 2.09 & 0.85 & 0.85 \\
0031 & 17.43 & 8196 & 2.08 & 0.80 & 0.85 \\
0030 & 15.85 & 8673 & 2.06 & 0.96 & 0.82 \\
0022 & 18.83 & 7870 & 2.11 & 0.65 & 0.87 \\
0021 & 15.57 & 8593 & 2.08 & 1.07 & 0.83 \\
0020 & 16.63 & 8152 & 2.10 & 0.78 & 0.86 \\
0011 & 17.15 & 8045 & 2.08 & 0.89 & 0.86 \\
0010 & 17.07 & 8166 & 2.11 & 1.00 & 0.85 \\
0000 & 12.61 & 8552 & 2.10 & 0.53 & 0.88 \\
\bottomrule
\end{tabular}


==> results/meta-llama/Llama-3.2-3B-Instruct/Julius/sample/control_table.tex <==
\begin{tabular}{rrrrr}
\toprule
tPPL() & N & Zipf & repl & DAvg \\
\midrule
17.99 & 26134 & 1.87 & 0.56 & 0.88 \\
\bottomrule
\end{tabular}


==> results/meta-llama/Llama-3.2-3B-Instruct/Julius/sample/gen_table.tex <==
\begin{tabular}{lrrrrr}
\toprule
scalings & tPPL() & N & Zipf & repl & DAvg \\
\midrule
0221 & 35.88 & 8591 & 2.00 & 1.61 & 0.74 \\
0220 & 38.57 & 8926 & 1.98 & 1.52 & 0.76 \\
0111 & 53.58 & 7712 & 2.14 & 0.71 & 0.87 \\
1111 & 38.76 & 7760 & 2.09 & 1.14 & 0.79 \\
0110 & 40.65 & 7850 & 2.10 & 1.31 & 0.82 \\
1110 & 54.93 & 7657 & 2.05 & 0.56 & 0.85 \\
0033 & 28.00 & 7676 & 2.13 & 0.71 & 0.86 \\
0032 & 28.98 & 7569 & 2.16 & 0.50 & 0.89 \\
0031 & 24.94 & 7726 & 2.23 & 0.71 & 0.88 \\
0030 & 28.98 & 8116 & 2.16 & 0.54 & 0.89 \\
0022 & 27.29 & 7672 & 2.18 & 0.54 & 0.89 \\
0021 & 28.71 & 8475 & 2.17 & 0.56 & 0.88 \\
0020 & 27.31 & 7601 & 2.20 & 0.48 & 0.89 \\
0011 & 23.15 & 8426 & 2.17 & 0.65 & 0.87 \\
0010 & 23.71 & 7994 & 2.18 & 0.69 & 0.89 \\
0000 & 14.67 & 8465 & 2.16 & 0.49 & 0.89 \\
\bottomrule
\end{tabular}


==> results/meta-llama/Llama-3.2-3B-Instruct/Todd/greedy/control_table.tex <==
\begin{tabular}{rrrrr}
\toprule
tPPL() & N & Zipf & repl & DAvg \\
\midrule
14.65 & 26186 & 1.81 & 0.62 & 0.88 \\
\bottomrule
\end{tabular}


==> results/meta-llama/Llama-3.2-3B-Instruct/Todd/greedy/gen_table.tex <==
\begin{tabular}{lrrrrr}
\toprule
scalings & tPPL() & N & Zipf & repl & DAvg \\
\midrule
0221 & 7.83 & 10002 & 1.73 & 2.51 & 0.49 \\
0220 & 7.78 & 10135 & 1.73 & 2.50 & 0.47 \\
0111 & 8.53 & 8790 & 1.78 & 2.15 & 0.58 \\
1111 & 8.53 & 8790 & 1.78 & 2.15 & 0.58 \\
0110 & 7.36 & 8923 & 1.78 & 2.26 & 0.55 \\
1110 & 7.36 & 8923 & 1.78 & 2.26 & 0.55 \\
0033 & 11.72 & 9238 & 2.04 & 1.84 & 0.73 \\
0032 & 12.33 & 9093 & 2.01 & 1.71 & 0.74 \\
0031 & 12.57 & 8760 & 2.02 & 1.59 & 0.75 \\
0030 & 12.82 & 8972 & 2.00 & 1.38 & 0.76 \\
0022 & 15.43 & 8418 & 2.03 & 1.25 & 0.80 \\
0021 & 15.27 & 8467 & 2.02 & 1.32 & 0.81 \\
0020 & 15.15 & 8223 & 2.06 & 1.37 & 0.81 \\
0011 & 17.09 & 7922 & 2.02 & 0.86 & 0.82 \\
0010 & 18.11 & 7957 & 2.05 & 0.80 & 0.84 \\
0000 & 12.61 & 8552 & 2.10 & 0.53 & 0.88 \\
\bottomrule
\end{tabular}


==> results/meta-llama/Llama-3.2-3B-Instruct/Todd/sample/control_table.tex <==
\begin{tabular}{rrrrr}
\toprule
tPPL() & N & Zipf & repl & DAvg \\
\midrule
18.80 & 25968 & 1.87 & 0.55 & 0.88 \\
\bottomrule
\end{tabular}


==> results/meta-llama/Llama-3.2-3B-Instruct/Todd/sample/gen_table.tex <==
\begin{tabular}{lrrrrr}
\toprule
scalings & tPPL() & N & Zipf & repl & DAvg \\
\midrule
0221 & 29.87 & 6706 & 1.93 & 0.82 & 0.81 \\
0220 & 25.37 & 7758 & 1.92 & 0.79 & 0.78 \\
0111 & 31.80 & 6801 & 1.93 & 0.60 & 0.83 \\
1111 & 44.58 & 6262 & 1.95 & 0.48 & 0.84 \\
0110 & 42.00 & 7046 & 1.95 & 0.52 & 0.83 \\
1110 & 41.85 & 6802 & 1.96 & 0.57 & 0.83 \\
0033 & 23.30 & 7939 & 2.10 & 0.67 & 0.87 \\
0032 & 23.11 & 8288 & 2.10 & 0.72 & 0.86 \\
0031 & 24.03 & 7958 & 2.10 & 0.69 & 0.86 \\
0030 & 25.76 & 7819 & 2.11 & 0.59 & 0.87 \\
0022 & 23.12 & 8146 & 2.09 & 1.19 & 0.84 \\
0021 & 26.55 & 8247 & 2.09 & 0.74 & 0.86 \\
0020 & 22.68 & 7939 & 2.14 & 0.99 & 0.86 \\
0011 & 27.33 & 7544 & 2.15 & 0.52 & 0.88 \\
0010 & 28.25 & 7635 & 2.18 & 0.52 & 0.89 \\
0000 & 15.26 & 8668 & 2.17 & 0.51 & 0.89 \\
\bottomrule
\end{tabular}


==> results/meta-llama/Llama-3.2-3B-Instruct/dooley/greedy/control_table.tex <==
\begin{tabular}{rrrrr}
\toprule
tPPL() & N & Zipf & repl & DAvg \\
\midrule
15.26 & 28915 & 1.81 & 0.67 & 0.85 \\
\bottomrule
\end{tabular}


==> results/meta-llama/Llama-3.2-3B-Instruct/dooley/greedy/gen_table.tex <==
\begin{tabular}{lrrrrr}
\toprule
scalings & tPPL() & N & Zipf & repl & DAvg \\
\midrule
0221 & 17.40 & 9424 & 1.86 & 1.89 & 0.62 \\
0220 & 16.89 & 9724 & 1.86 & 1.98 & 0.61 \\
0111 & 19.23 & 8848 & 1.88 & 1.28 & 0.67 \\
1111 & 19.23 & 8848 & 1.88 & 1.28 & 0.67 \\
0110 & 21.20 & 8593 & 1.89 & 1.16 & 0.68 \\
1110 & 21.20 & 8593 & 1.89 & 1.16 & 0.68 \\
0033 & 18.94 & 8154 & 2.08 & 0.63 & 0.85 \\
0032 & 18.83 & 8081 & 2.08 & 0.62 & 0.85 \\
0031 & 19.06 & 8149 & 2.07 & 0.62 & 0.85 \\
0030 & 18.64 & 8126 & 2.07 & 0.62 & 0.84 \\
0022 & 17.85 & 7760 & 2.08 & 0.66 & 0.86 \\
0021 & 16.81 & 7846 & 2.08 & 0.95 & 0.85 \\
0020 & 16.41 & 7837 & 2.09 & 0.96 & 0.85 \\
0011 & 18.20 & 7543 & 2.08 & 0.60 & 0.84 \\
0010 & 18.12 & 7519 & 2.09 & 0.59 & 0.84 \\
0000 & 12.61 & 8552 & 2.10 & 0.53 & 0.88 \\
\bottomrule
\end{tabular}


==> results/meta-llama/Llama-3.2-3B-Instruct/dooley/sample/control_table.tex <==
\begin{tabular}{rrrrr}
\toprule
tPPL() & N & Zipf & repl & DAvg \\
\midrule
19.24 & 28327 & 1.89 & 0.58 & 0.88 \\
\bottomrule
\end{tabular}


==> results/meta-llama/Llama-3.2-3B-Instruct/dooley/sample/gen_table.tex <==
\begin{tabular}{lrrrrr}
\toprule
scalings & tPPL() & N & Zipf & repl & DAvg \\
\midrule
0221 & 52.47 & 6949 & 2.10 & 0.54 & 0.87 \\
0220 & 52.62 & 7137 & 2.10 & 0.53 & 0.87 \\
0111 & 49.88 & 6455 & 2.14 & 0.59 & 0.85 \\
1111 & 58.94 & 6112 & 2.13 & 0.66 & 0.87 \\
0110 & 47.26 & 7309 & 2.07 & 0.79 & 0.85 \\
1110 & 44.37 & 6831 & 2.11 & 0.70 & 0.86 \\
0033 & 25.95 & 7890 & 2.15 & 0.54 & 0.89 \\
0032 & 27.28 & 7795 & 2.16 & 0.95 & 0.87 \\
0031 & 26.85 & 7955 & 2.19 & 0.63 & 0.87 \\
0030 & 24.10 & 7551 & 2.18 & 0.67 & 0.87 \\
0022 & 28.38 & 7636 & 2.17 & 0.51 & 0.89 \\
0021 & 26.01 & 8114 & 2.15 & 0.53 & 0.88 \\
0020 & 24.64 & 7858 & 2.17 & 0.57 & 0.86 \\
0011 & 26.59 & 7061 & 2.17 & 0.45 & 0.90 \\
0010 & 25.26 & 7644 & 2.20 & 0.52 & 0.88 \\
0000 & 15.39 & 8322 & 2.16 & 0.52 & 0.89 \\
\bottomrule
\end{tabular}


==> results/meta-llama/Llama-3.2-3B-Instruct/remus/greedy/control_table.tex <==
\begin{tabular}{rrrrr}
\toprule
tPPL() & N & Zipf & repl & DAvg \\
\midrule
15.35 & 26579 & 1.76 & 0.59 & 0.87 \\
\bottomrule
\end{tabular}


==> results/meta-llama/Llama-3.2-3B-Instruct/remus/greedy/gen_table.tex <==
\begin{tabular}{lrrrrr}
\toprule
scalings & tPPL() & N & Zipf & repl & DAvg \\
\midrule
0221 & 17.04 & 8705 & 1.90 & 1.44 & 0.67 \\
0220 & 16.19 & 8833 & 1.89 & 1.45 & 0.64 \\
0111 & 16.58 & 8461 & 1.94 & 1.51 & 0.69 \\
1111 & 16.58 & 8461 & 1.94 & 1.51 & 0.69 \\
0110 & 18.71 & 7828 & 2.00 & 1.30 & 0.74 \\
1110 & 18.71 & 7828 & 2.00 & 1.30 & 0.74 \\
0033 & 17.85 & 8382 & 2.05 & 1.18 & 0.80 \\
0032 & 19.65 & 8103 & 2.02 & 0.98 & 0.80 \\
0031 & 19.15 & 8155 & 2.04 & 1.04 & 0.80 \\
0030 & 16.37 & 8851 & 2.02 & 1.26 & 0.76 \\
0022 & 21.77 & 7873 & 2.11 & 0.87 & 0.84 \\
0021 & 20.43 & 8217 & 2.07 & 1.07 & 0.82 \\
0020 & 20.59 & 8348 & 2.06 & 1.09 & 0.81 \\
0011 & 18.27 & 8007 & 2.04 & 0.97 & 0.80 \\
0010 & 17.61 & 7672 & 2.04 & 0.99 & 0.80 \\
0000 & 12.61 & 8552 & 2.10 & 0.53 & 0.88 \\
\bottomrule
\end{tabular}


==> results/meta-llama/Llama-3.2-3B-Instruct/remus/sample/control_table.tex <==
\begin{tabular}{rrrrr}
\toprule
tPPL() & N & Zipf & repl & DAvg \\
\midrule
19.86 & 28120 & 1.83 & 0.57 & 0.88 \\
\bottomrule
\end{tabular}


==> results/meta-llama/Llama-3.2-3B-Instruct/remus/sample/gen_table.tex <==
\begin{tabular}{lrrrrr}
\toprule
scalings & tPPL() & N & Zipf & repl & DAvg \\
\midrule
0221 & 47.37 & 7402 & 2.11 & 0.78 & 0.85 \\
0220 & 44.14 & 7652 & 2.08 & 1.02 & 0.82 \\
0111 & 61.87 & 7865 & 2.07 & 0.50 & 0.86 \\
1111 & 55.09 & 8475 & 2.07 & 0.70 & 0.85 \\
0110 & 46.55 & 7424 & 2.13 & 0.73 & 0.85 \\
1110 & 54.94 & 8004 & 2.09 & 0.62 & 0.85 \\
0033 & 29.04 & 8045 & 2.14 & 0.86 & 0.84 \\
0032 & 30.58 & 7900 & 2.17 & 0.85 & 0.88 \\
0031 & 28.99 & 7509 & 2.13 & 0.69 & 0.86 \\
0030 & 31.07 & 8032 & 2.12 & 0.58 & 0.86 \\
0022 & 31.36 & 7861 & 2.14 & 0.74 & 0.86 \\
0021 & 32.05 & 7744 & 2.18 & 0.73 & 0.88 \\
0020 & 34.62 & 7826 & 2.18 & 0.54 & 0.88 \\
0011 & 33.16 & 7357 & 2.21 & 0.48 & 0.88 \\
0010 & 31.51 & 7542 & 2.16 & 0.59 & 0.88 \\
0000 & 14.84 & 8685 & 2.16 & 0.53 & 0.89 \\
\bottomrule
\end{tabular}


==> results/mistralai/Mistral-7B-Instruct-v0.2/Biglow/greedy/control_table.tex <==
\begin{tabular}{rrrrr}
\toprule
tPPL() & N & Zipf & repl & DAvg \\
\midrule
15.94 & 33392 & 1.78 & 0.65 & 0.87 \\
\bottomrule
\end{tabular}


==> results/mistralai/Mistral-7B-Instruct-v0.2/Biglow/greedy/gen_table.tex <==
\begin{tabular}{lrrrrr}
\toprule
scalings & tPPL() & N & Zipf & repl & DAvg \\
\midrule
0221 & 24.49 & 14008 & 1.92 & 4.19 & 0.56 \\
0220 & 24.54 & 14045 & 1.92 & 4.25 & 0.55 \\
0111 & 35.31 & 13631 & 1.94 & 3.43 & 0.62 \\
1111 & 35.31 & 13631 & 1.94 & 3.43 & 0.62 \\
0110 & 38.04 & 13803 & 1.93 & 3.48 & 0.63 \\
1110 & 38.04 & 13803 & 1.93 & 3.48 & 0.63 \\
0033 & 42.47 & 11469 & 2.04 & 1.39 & 0.81 \\
0032 & 44.41 & 11411 & 2.03 & 1.18 & 0.82 \\
0031 & 44.73 & 11399 & 2.05 & 1.15 & 0.83 \\
0030 & 42.20 & 11438 & 2.03 & 1.17 & 0.82 \\
0022 & 44.62 & 11077 & 2.02 & 1.19 & 0.80 \\
0021 & 43.51 & 11196 & 2.02 & 1.14 & 0.81 \\
0020 & 43.01 & 11175 & 2.01 & 1.14 & 0.81 \\
0011 & 45.45 & 11126 & 2.03 & 0.88 & 0.82 \\
0010 & 48.16 & 11067 & 2.01 & 0.87 & 0.82 \\
0000 & 14.10 & 9941 & 2.05 & 0.58 & 0.87 \\
\bottomrule
\end{tabular}


==> results/mistralai/Mistral-7B-Instruct-v0.2/Biglow/sample/control_table.tex <==
\begin{tabular}{rrrrr}
\toprule
tPPL() & N & Zipf & repl & DAvg \\
\midrule
22.20 & 32830 & 1.85 & 0.61 & 0.89 \\
\bottomrule
\end{tabular}


==> results/mistralai/Mistral-7B-Instruct-v0.2/Biglow/sample/gen_table.tex <==
\begin{tabular}{lrrrrr}
\toprule
scalings & tPPL() & N & Zipf & repl & DAvg \\
\midrule
0221 & 61.06 & 13982 & 2.00 & 3.22 & 0.67 \\
0220 & 67.89 & 13402 & 1.99 & 2.80 & 0.71 \\
0111 & 79.19 & 13511 & 2.03 & 2.56 & 0.72 \\
1111 & 71.70 & 13602 & 2.03 & 2.86 & 0.73 \\
0110 & 74.11 & 13331 & 2.00 & 2.46 & 0.71 \\
1110 & 84.00 & 13014 & 1.99 & 2.13 & 0.73 \\
0033 & 81.42 & 11528 & 2.09 & 0.80 & 0.86 \\
0032 & 88.46 & 11545 & 2.10 & 0.78 & 0.85 \\
0031 & 77.01 & 11580 & 2.11 & 0.77 & 0.86 \\
0030 & 79.46 & 11271 & 2.08 & 0.68 & 0.86 \\
0022 & 71.21 & 11132 & 2.11 & 0.72 & 0.88 \\
0021 & 68.28 & 11233 & 2.12 & 0.63 & 0.88 \\
0020 & 74.91 & 11482 & 2.12 & 0.71 & 0.86 \\
0011 & 69.02 & 10975 & 2.12 & 0.58 & 0.88 \\
0010 & 76.35 & 11175 & 2.10 & 0.56 & 0.88 \\
0000 & 17.23 & 9790 & 2.11 & 0.58 & 0.88 \\
\bottomrule
\end{tabular}


==> results/mistralai/Mistral-7B-Instruct-v0.2/Huck/greedy/control_table.tex <==
\begin{tabular}{rrrrr}
\toprule
tPPL() & N & Zipf & repl & DAvg \\
\midrule
16.45 & 33308 & 1.78 & 0.71 & 0.87 \\
\bottomrule
\end{tabular}


==> results/mistralai/Mistral-7B-Instruct-v0.2/Huck/greedy/gen_table.tex <==
\begin{tabular}{lrrrrr}
\toprule
scalings & tPPL() & N & Zipf & repl & DAvg \\
\midrule
0221 & 23.76 & 11257 & 1.96 & 2.02 & 0.68 \\
0220 & 25.03 & 11260 & 1.98 & 1.96 & 0.69 \\
0111 & 29.51 & 11266 & 1.98 & 1.57 & 0.68 \\
1111 & 29.51 & 11266 & 1.98 & 1.57 & 0.68 \\
0110 & 25.41 & 11378 & 1.99 & 1.82 & 0.66 \\
1110 & 25.41 & 11378 & 1.99 & 1.82 & 0.66 \\
0033 & 22.36 & 10291 & 2.05 & 1.03 & 0.84 \\
0032 & 23.62 & 10259 & 2.05 & 0.98 & 0.84 \\
0031 & 23.30 & 10303 & 2.06 & 0.95 & 0.84 \\
0030 & 23.56 & 10358 & 2.06 & 0.97 & 0.84 \\
0022 & 24.85 & 10162 & 2.04 & 0.78 & 0.86 \\
0021 & 24.78 & 10122 & 2.05 & 0.81 & 0.85 \\
0020 & 23.77 & 10211 & 2.05 & 0.98 & 0.84 \\
0011 & 28.56 & 10084 & 2.03 & 0.71 & 0.86 \\
0010 & 29.02 & 10278 & 2.03 & 0.72 & 0.85 \\
0000 & 14.10 & 9941 & 2.05 & 0.58 & 0.87 \\
\bottomrule
\end{tabular}


==> results/mistralai/Mistral-7B-Instruct-v0.2/Huck/sample/control_table.tex <==
\begin{tabular}{rrrrr}
\toprule
tPPL() & N & Zipf & repl & DAvg \\
\midrule
22.06 & 33501 & 1.84 & 0.60 & 0.88 \\
\bottomrule
\end{tabular}


==> results/mistralai/Mistral-7B-Instruct-v0.2/Huck/sample/gen_table.tex <==
\begin{tabular}{lrrrrr}
\toprule
scalings & tPPL() & N & Zipf & repl & DAvg \\
\midrule
0221 & 51.19 & 11259 & 2.08 & 1.26 & 0.80 \\
0220 & 52.23 & 11055 & 2.06 & 1.03 & 0.80 \\
0111 & 64.90 & 11237 & 2.02 & 0.77 & 0.83 \\
1111 & 65.97 & 10968 & 2.05 & 0.86 & 0.81 \\
0110 & 47.40 & 11407 & 2.09 & 1.19 & 0.76 \\
1110 & 50.28 & 11206 & 2.07 & 1.22 & 0.78 \\
0033 & 33.59 & 10176 & 2.12 & 0.93 & 0.86 \\
0032 & 35.26 & 10520 & 2.10 & 0.77 & 0.86 \\
0031 & 36.97 & 10720 & 2.11 & 0.73 & 0.86 \\
0030 & 39.64 & 10708 & 2.09 & 0.76 & 0.86 \\
0022 & 35.72 & 10111 & 2.09 & 0.76 & 0.86 \\
0021 & 39.00 & 10206 & 2.09 & 0.68 & 0.86 \\
0020 & 39.47 & 10232 & 2.09 & 0.65 & 0.87 \\
0011 & 37.59 & 10476 & 2.10 & 0.72 & 0.87 \\
0010 & 33.59 & 10186 & 2.12 & 0.71 & 0.87 \\
0000 & 18.50 & 9634 & 2.15 & 0.56 & 0.89 \\
\bottomrule
\end{tabular}


==> results/mistralai/Mistral-7B-Instruct-v0.2/Julius/greedy/control_table.tex <==
\begin{tabular}{rrrrr}
\toprule
tPPL() & N & Zipf & repl & DAvg \\
\midrule
15.17 & 33330 & 1.80 & 0.66 & 0.88 \\
\bottomrule
\end{tabular}


==> results/mistralai/Mistral-7B-Instruct-v0.2/Julius/greedy/gen_table.tex <==
\begin{tabular}{lrrrrr}
\toprule
scalings & tPPL() & N & Zipf & repl & DAvg \\
\midrule
0221 & 79.21 & 11562 & 1.95 & 0.99 & 0.74 \\
0220 & 79.66 & 11262 & 1.93 & 0.99 & 0.75 \\
0111 & 76.27 & 11565 & 1.97 & 0.97 & 0.75 \\
1111 & 76.27 & 11565 & 1.97 & 0.97 & 0.75 \\
0110 & 82.43 & 11347 & 1.97 & 0.91 & 0.77 \\
1110 & 82.43 & 11347 & 1.97 & 0.91 & 0.77 \\
0033 & 48.05 & 10230 & 2.04 & 1.48 & 0.83 \\
0032 & 49.80 & 10242 & 2.04 & 1.61 & 0.83 \\
0031 & 46.68 & 10011 & 2.03 & 1.57 & 0.83 \\
0030 & 40.54 & 10132 & 2.04 & 2.40 & 0.79 \\
0022 & 45.10 & 10187 & 2.04 & 1.45 & 0.84 \\
0021 & 39.92 & 10280 & 2.05 & 1.46 & 0.84 \\
0020 & 40.25 & 10275 & 2.03 & 1.44 & 0.83 \\
0011 & 40.86 & 10363 & 2.03 & 0.83 & 0.85 \\
0010 & 44.42 & 10423 & 2.05 & 0.70 & 0.85 \\
0000 & 14.10 & 9941 & 2.05 & 0.58 & 0.87 \\
\bottomrule
\end{tabular}


==> results/mistralai/Mistral-7B-Instruct-v0.2/Julius/sample/control_table.tex <==
\begin{tabular}{rrrrr}
\toprule
tPPL() & N & Zipf & repl & DAvg \\
\midrule
20.65 & 33225 & 1.84 & 0.61 & 0.89 \\
\bottomrule
\end{tabular}


==> results/mistralai/Mistral-7B-Instruct-v0.2/Julius/sample/gen_table.tex <==
\begin{tabular}{lrrrrr}
\toprule
scalings & tPPL() & N & Zipf & repl & DAvg \\
\midrule
0221 & 148.68 & 11288 & 2.02 & 0.86 & 0.83 \\
0220 & 160.40 & 11635 & 2.00 & 0.87 & 0.83 \\
0111 & 124.46 & 11188 & 2.02 & 0.80 & 0.83 \\
1111 & 159.66 & 11474 & 2.00 & 0.57 & 0.84 \\
0110 & 154.42 & 11399 & 2.00 & 0.57 & 0.85 \\
1110 & 140.28 & 11425 & 2.03 & 0.79 & 0.85 \\
0033 & 82.56 & 10516 & 2.10 & 0.60 & 0.89 \\
0032 & 84.51 & 10320 & 2.14 & 0.93 & 0.88 \\
0031 & 76.96 & 10714 & 2.12 & 0.78 & 0.88 \\
0030 & 73.66 & 10458 & 2.13 & 0.54 & 0.88 \\
0022 & 70.59 & 10658 & 2.13 & 0.56 & 0.89 \\
0021 & 62.58 & 10642 & 2.14 & 1.39 & 0.86 \\
0020 & 74.62 & 10626 & 2.12 & 0.53 & 0.89 \\
0011 & 72.63 & 10297 & 2.13 & 0.56 & 0.88 \\
0010 & 69.49 & 10607 & 2.14 & 0.97 & 0.87 \\
0000 & 17.06 & 9956 & 2.10 & 0.57 & 0.88 \\
\bottomrule
\end{tabular}


==> results/mistralai/Mistral-7B-Instruct-v0.2/Todd/greedy/control_table.tex <==
\begin{tabular}{rrrrr}
\toprule
tPPL() & N & Zipf & repl & DAvg \\
\midrule
15.98 & 33355 & 1.77 & 0.66 & 0.87 \\
\bottomrule
\end{tabular}


==> results/mistralai/Mistral-7B-Instruct-v0.2/Todd/greedy/gen_table.tex <==
\begin{tabular}{lrrrrr}
\toprule
scalings & tPPL() & N & Zipf & repl & DAvg \\
\midrule
0221 & 31.45 & 11538 & 1.83 & 1.52 & 0.62 \\
0220 & 32.08 & 11386 & 1.86 & 1.52 & 0.64 \\
0111 & 39.19 & 11529 & 1.87 & 1.12 & 0.69 \\
1111 & 39.19 & 11529 & 1.87 & 1.12 & 0.69 \\
0110 & 42.59 & 11264 & 1.89 & 1.10 & 0.72 \\
1110 & 42.59 & 11264 & 1.89 & 1.10 & 0.72 \\
0033 & 34.08 & 10308 & 2.00 & 1.04 & 0.83 \\
0032 & 32.01 & 10587 & 2.00 & 1.05 & 0.82 \\
0031 & 33.82 & 10479 & 2.02 & 1.05 & 0.82 \\
0030 & 33.24 & 10513 & 2.01 & 1.05 & 0.82 \\
0022 & 30.18 & 10479 & 2.03 & 1.31 & 0.80 \\
0021 & 32.00 & 10545 & 2.03 & 1.16 & 0.81 \\
0020 & 35.42 & 10489 & 2.02 & 1.03 & 0.82 \\
0011 & 34.51 & 10353 & 2.01 & 0.86 & 0.84 \\
0010 & 34.72 & 10265 & 2.02 & 0.85 & 0.85 \\
0000 & 14.10 & 9941 & 2.05 & 0.58 & 0.87 \\
\bottomrule
\end{tabular}


==> results/mistralai/Mistral-7B-Instruct-v0.2/Todd/sample/control_table.tex <==
\begin{tabular}{rrrrr}
\toprule
tPPL() & N & Zipf & repl & DAvg \\
\midrule
21.47 & 32455 & 1.83 & 0.59 & 0.89 \\
\bottomrule
\end{tabular}


==> results/mistralai/Mistral-7B-Instruct-v0.2/Todd/sample/gen_table.tex <==
\begin{tabular}{lrrrrr}
\toprule
scalings & tPPL() & N & Zipf & repl & DAvg \\
\midrule
0221 & 69.43 & 11698 & 1.95 & 0.75 & 0.81 \\
0220 & 69.83 & 11557 & 1.99 & 0.79 & 0.82 \\
0111 & 75.14 & 11468 & 1.98 & 0.67 & 0.84 \\
1111 & 79.22 & 11516 & 2.01 & 0.66 & 0.83 \\
0110 & 89.15 & 11444 & 1.98 & 0.60 & 0.84 \\
1110 & 80.32 & 11289 & 1.99 & 0.68 & 0.84 \\
0033 & 50.16 & 10699 & 2.07 & 0.78 & 0.86 \\
0032 & 47.78 & 10582 & 2.09 & 1.03 & 0.85 \\
0031 & 54.16 & 10683 & 2.11 & 0.71 & 0.86 \\
0030 & 54.88 & 10336 & 2.12 & 0.71 & 0.85 \\
0022 & 60.03 & 10768 & 2.08 & 0.64 & 0.87 \\
0021 & 52.41 & 10107 & 2.10 & 0.82 & 0.86 \\
0020 & 58.95 & 10449 & 2.09 & 0.67 & 0.87 \\
0011 & 55.55 & 10777 & 2.10 & 0.60 & 0.88 \\
0010 & 61.68 & 10590 & 2.07 & 0.57 & 0.88 \\
0000 & 17.17 & 9871 & 2.11 & 0.59 & 0.88 \\
\bottomrule
\end{tabular}


==> results/mistralai/Mistral-7B-Instruct-v0.2/dooley/greedy/control_table.tex <==
\begin{tabular}{rrrrr}
\toprule
tPPL() & N & Zipf & repl & DAvg \\
\midrule
17.58 & 33516 & 1.80 & 0.67 & 0.87 \\
\bottomrule
\end{tabular}


==> results/mistralai/Mistral-7B-Instruct-v0.2/dooley/greedy/gen_table.tex <==
\begin{tabular}{lrrrrr}
\toprule
scalings & tPPL() & N & Zipf & repl & DAvg \\
\midrule
0221 & 59.82 & 10893 & 2.03 & 0.95 & 0.81 \\
0220 & 58.44 & 10883 & 2.02 & 0.96 & 0.81 \\
0111 & 69.48 & 11090 & 2.02 & 0.91 & 0.82 \\
1111 & 69.48 & 11090 & 2.02 & 0.91 & 0.82 \\
0110 & 70.08 & 11079 & 2.02 & 0.89 & 0.81 \\
1110 & 70.08 & 11079 & 2.02 & 0.89 & 0.81 \\
0033 & 29.62 & 10504 & 2.03 & 0.75 & 0.83 \\
0032 & 29.87 & 10414 & 2.02 & 0.75 & 0.83 \\
0031 & 28.81 & 10387 & 2.03 & 0.76 & 0.83 \\
0030 & 28.71 & 10395 & 2.03 & 0.76 & 0.83 \\
0022 & 26.91 & 10425 & 2.05 & 0.75 & 0.84 \\
0021 & 25.91 & 10373 & 2.04 & 0.75 & 0.83 \\
0020 & 25.92 & 10418 & 2.05 & 0.75 & 0.83 \\
0011 & 28.69 & 10142 & 2.05 & 0.76 & 0.85 \\
0010 & 28.51 & 10055 & 2.06 & 0.75 & 0.86 \\
0000 & 14.10 & 9941 & 2.05 & 0.58 & 0.87 \\
\bottomrule
\end{tabular}


==> results/mistralai/Mistral-7B-Instruct-v0.2/dooley/sample/control_table.tex <==
\begin{tabular}{rrrrr}
\toprule
tPPL() & N & Zipf & repl & DAvg \\
\midrule
25.50 & 33398 & 1.86 & 0.62 & 0.88 \\
\bottomrule
\end{tabular}


==> results/mistralai/Mistral-7B-Instruct-v0.2/dooley/sample/gen_table.tex <==
\begin{tabular}{lrrrrr}
\toprule
scalings & tPPL() & N & Zipf & repl & DAvg \\
\midrule
0221 & 101.11 & 11114 & 2.11 & 0.88 & 0.85 \\
0220 & 114.33 & 11330 & 2.09 & 0.83 & 0.85 \\
0111 & 125.46 & 11288 & 2.07 & 0.69 & 0.86 \\
1111 & 117.32 & 11193 & 2.11 & 0.72 & 0.87 \\
0110 & 124.31 & 10988 & 2.10 & 0.69 & 0.88 \\
1110 & 119.28 & 11081 & 2.08 & 0.69 & 0.87 \\
0033 & 40.70 & 10504 & 2.12 & 0.61 & 0.88 \\
0032 & 42.64 & 10711 & 2.12 & 0.63 & 0.87 \\
0031 & 43.03 & 10222 & 2.11 & 0.64 & 0.88 \\
0030 & 45.13 & 10651 & 2.12 & 0.58 & 0.88 \\
0022 & 44.00 & 10492 & 2.13 & 0.59 & 0.88 \\
0021 & 40.93 & 10299 & 2.12 & 0.58 & 0.87 \\
0020 & 46.46 & 10481 & 2.15 & 0.57 & 0.89 \\
0011 & 38.93 & 10751 & 2.12 & 0.61 & 0.88 \\
0010 & 42.90 & 10099 & 2.15 & 0.72 & 0.88 \\
0000 & 18.05 & 9702 & 2.16 & 0.57 & 0.89 \\
\bottomrule
\end{tabular}


==> results/mistralai/Mistral-7B-Instruct-v0.2/remus/greedy/control_table.tex <==
\begin{tabular}{rrrrr}
\toprule
tPPL() & N & Zipf & repl & DAvg \\
\midrule
19.19 & 33825 & 1.77 & 0.72 & 0.86 \\
\bottomrule
\end{tabular}


==> results/mistralai/Mistral-7B-Instruct-v0.2/remus/greedy/gen_table.tex <==
\begin{tabular}{lrrrrr}
\toprule
scalings & tPPL() & N & Zipf & repl & DAvg \\
\midrule
0221 & 42.30 & 11087 & 1.99 & 1.48 & 0.74 \\
0220 & 39.74 & 11173 & 1.98 & 2.01 & 0.72 \\
0111 & 41.34 & 11023 & 2.01 & 1.62 & 0.74 \\
1111 & 41.34 & 11023 & 2.01 & 1.62 & 0.74 \\
0110 & 37.73 & 11093 & 1.99 & 1.71 & 0.73 \\
1110 & 37.73 & 11093 & 1.99 & 1.71 & 0.73 \\
0033 & 31.58 & 9998 & 2.02 & 1.25 & 0.82 \\
0032 & 34.56 & 10052 & 2.06 & 0.89 & 0.83 \\
0031 & 33.03 & 10418 & 2.03 & 1.25 & 0.81 \\
0030 & 32.86 & 10134 & 2.06 & 1.26 & 0.81 \\
0022 & 35.65 & 10149 & 2.07 & 0.84 & 0.84 \\
0021 & 35.82 & 10131 & 2.06 & 0.83 & 0.83 \\
0020 & 34.11 & 10149 & 2.05 & 0.84 & 0.83 \\
0011 & 34.08 & 9970 & 2.07 & 0.83 & 0.84 \\
0010 & 34.85 & 9879 & 2.07 & 0.83 & 0.84 \\
0000 & 14.10 & 9941 & 2.05 & 0.58 & 0.87 \\
\bottomrule
\end{tabular}


==> results/mistralai/Mistral-7B-Instruct-v0.2/remus/sample/control_table.tex <==
\begin{tabular}{rrrrr}
\toprule
tPPL() & N & Zipf & repl & DAvg \\
\midrule
28.04 & 33507 & 1.82 & 0.63 & 0.88 \\
\bottomrule
\end{tabular}


==> results/mistralai/Mistral-7B-Instruct-v0.2/remus/sample/gen_table.tex <==
\begin{tabular}{lrrrrr}
\toprule
scalings & tPPL() & N & Zipf & repl & DAvg \\
\midrule
0221 & 87.69 & 11172 & 2.08 & 1.02 & 0.81 \\
0220 & 97.38 & 11171 & 2.05 & 0.74 & 0.84 \\
0111 & 87.55 & 11210 & 2.07 & 1.08 & 0.81 \\
1111 & 86.61 & 10928 & 2.05 & 0.88 & 0.82 \\
0110 & 92.08 & 10885 & 2.10 & 0.86 & 0.83 \\
1110 & 108.04 & 10695 & 2.07 & 0.74 & 0.85 \\
0033 & 57.29 & 10308 & 2.13 & 0.89 & 0.87 \\
0032 & 57.21 & 10794 & 2.10 & 0.85 & 0.84 \\
0031 & 57.65 & 10469 & 2.13 & 0.59 & 0.88 \\
0030 & 58.60 & 10401 & 2.13 & 0.69 & 0.88 \\
0022 & 62.44 & 10799 & 2.11 & 0.59 & 0.88 \\
0021 & 55.15 & 10621 & 2.12 & 0.71 & 0.86 \\
0020 & 63.76 & 10668 & 2.09 & 0.55 & 0.88 \\
0011 & 60.68 & 10577 & 2.12 & 0.55 & 0.88 \\
0010 & 57.43 & 10650 & 2.13 & 0.58 & 0.87 \\
0000 & 17.25 & 10144 & 2.11 & 0.56 & 0.88 \\
\bottomrule
\end{tabular}


==> results/target_table.tex <==
\begin{tabular}{lrrrrrr}
\toprule
name & p & N & Zipf & repl & D_avg & D_full \\
\midrule
openai-community/gpt2-large & 41.01 & 12456693 & 1.24 & 0.89 & 0.72 & 0.29 \\
\bottomrule
\end{tabular}

